Interdependent Public Projects

In the interdependent values (IDV) model introduced by Milgrom and Weber [1982], agents have private signals that capture their information about different social alternatives, and the valuation of every agent is a function of all agent signals. While interdependence has been mainly studied for auctions, it is extremely relevant for a large variety of social choice settings, including the canonical setting of public projects. The IDV model is very challenging relative to standard independent private values, and welfare guarantees have been achieved through two alternative conditions known as {\em single-crossing} and {\em submodularity over signals (SOS)}. In either case, the existing theory falls short of solving the public projects setting. Our contribution is twofold: (i) We give a workable characterization of truthfulness for IDV public projects for the largest class of valuations for which such a characterization exists, and term this class \emph{decomposable valuations}; (ii) We provide possibility and impossibility results for welfare approximation in public projects with SOS valuations. Our main impossibility result is that, in contrast to auctions, no universally truthful mechanism performs better for public projects with SOS valuations than choosing a project at random. Our main positive result applies to {\em excludable} public projects with SOS, for which we establish a constant factor approximation similar to auctions. Our results suggest that exclusion may be a key tool for achieving welfare guarantees in the IDV model.

==> arXiv version/approximation.tex <==
\section{Approximate Welfare Maximization in Public Projects}
% No strong single crossing 
%\section{The Limits of SOS: Impossibility without Exclusion}
\label{sec:approximation}
 
%\inbal{We decided to move here SOS and impossibility without it as preliminaries for the section}
 
%%%\outline{Impossibility result -- without excludability+WMON cannot do better than choosing a project at random (even for linear with binary signals). Choosing a project at random is WMON. %Excludability is well-established ``club goods''. 
 %If there is excludability + SOS + separability then there is a 4-approximation. 
 %SOS is necessary. 
%%%Also mention that even if values depend on at most $2$ signals~\cite[cf.][]{EGZ22}. %Can we leverage this to say that ``exclusion'' is necessary for auctions too? 
%%%Motivating example: Need to exclude conference PC from paper selection?} 
%\todo{present the impossibility before the approximation result}
            %\dnote{DM: an example where for the OG setting with SOS and separability we still can't do better than a 1/m approximation for any universally truthful mechanism.}

In this section we focus on the public projects setting with IDV valuations, and study truthful mechanisms that get approximately-optimal social welfare. 
Recall that we are given $n$ agents and $m$ projects, and we want to allocate up to $k$ projects. We observe in Section~\ref{sub:reduction} that even with $k= 1$, the public projects setting is rich enough to capture any general social choice setting (computation aside). This is because, given any social choice setting with IDV valuations $(n,\mathcal{S},\mathcal{A},\vprofile)$, we can consider a public project setting where each alternative $a\in \mathcal{A}$ has a corresponding project (that is, we have $n$ agents, $m = |\mathcal{A}|$ projects, and wish to choose a single project/alternative). %\divya{maybe I should move this to somewhere else}


By Proposition~\ref{prop:linear-characterization} it holds that for decomposable valuations, strong single-crossing is both a necessary and sufficient condition to achieve optimal social welfare truthfully. {We shall show in Section~\ref{sec:impossibility-result} that, in the absence of strong single-crossing, and even when restricting our attention to decomposable valuations (or even \linear valuations), there are strong impossibility results for obtaining non-trivial welfare guarantees truthfully.}

In Section~\ref{sub:exclusion-to-rescue} we apply a known tool for truthfulness -- excluding agents. Intuitively, excluded agents have no stake in the outcome and thus would report truthfully. 
Shifting focus to a variant of public goods that allows agent exclusion enables us to circumvent the impossibility result of Theorem~\ref{thm:lower-bound}.

%\subsection{Section Preliminaries: SOS and Separable SOS}

%\vspace{1ex}
%\noindent{\bf SOS and separable SOS.} 
\paragraph{Section preliminaries.}
We revisit well-studied conditions on valuation functions in the interdependent setting. In the IDV auctions setting, these have been useful for  obtaining approximately-optimal welfare truthfully even when single-crossing %conditions do not hold.  
{does not hold}. The definitions below are adapted from~\cite{EFFGK19}.

\begin{definition}[Submodular-over-signals valuations]
A valuation function $v: \mathcal{A}\times\mathcal{S} \rightarrow \reals^+$ satisfies {\em submodularity over signals} (SOS) if for all $a\in\mathcal{A},\;\profile,\,\profile'\in \mathcal{S}$ and $i \in [n]$, where $\profile'$ is coordinate wise larger or equal to $\profile$ it holds that
\[
    v(a;s'_i,\sminus) - v(a;\profile) \ge v(a;\profile') - v(a; s_i,\profile'_{-i})
\]
%\michal{Would it make sense to use bold instead of the vector arrow? if so, we should do a global change. Somehow, the combination of the arrow and the apostrophe looks quite bad.}
\end{definition}
 
\begin{definition}[Separable SOS valuations]
For each agent $i$, a valuation function $v_i: \mathcal{A}\times\mathcal{S} \rightarrow \reals^+$ is  {\em separable SOS} if there exist functions $g_{-i}: \mathcal{A}\times\mathcal{S}_{-i} \rightarrow \reals^+$ and $h_i: \mathcal{A}\times S_i \rightarrow \reals^+$ such that 
\[
    v_i(a;\profile) = h_i(a;s_i) + g_{-i}(a; \profile_{-i}) ,
\]
%
 where $h_i(\cdot)$ and $g_{-i}(\cdot)$ are both weakly increasing and $g_{-i}(\cdot)$ is an SOS function.
\end{definition}

%Observe that any separable SOS valuation $v_i$ is a decomposable valuation. That is, seperable SOS valuations are a subclass of decomposable valuations.


% Observe that the lower bound holds even when valuations are separable SOS because Example~\ref{eg:lower-bound-1/n} linear valuations which are both Separable and SOS!
% \michal{what's the context of this comment?} \avi{We moved this section around... It used to be after Section 4.3.}


% Preliminary Result: 
\subsection{Reducing Auctions to Public Projects and Impossibility Implications}
\label{sub:reduction}

In this section we show that known impossibility results from IDV single-item auctions carry over to IDV public projects via a simple reduction.


%\vspace{1ex}
%\noindent{\bf Single-item auctions with IDV.}

{
A single-item auction instance is given by $(n, \mathcal{S},\mathcal{A},\vprofile)$, where a single item needs to be allocated to one of $n$ agents, $\mathcal{A} = [n]$ is the set of possible outcomes (outcome $i$ denotes an allocation to agent $i$), every agent $i$ has a valuation $v_i: \mathcal{S} \rightarrow \reals^+$, where the value of agent $i$ for winning the item under signal profile  $\profile$ is $v_i(\profile)$, and $0$ otherwise (i.e., if $i$ is not the winner).
}
%Given any instance $(n, \mathcal{S},\mathcal{A},\vprofile)$ in the single-item auctions setting, with $n$ agents, a single item that needs to be allocated to one of the agents (i.e, $\mathcal{A} = [n]$); 
%More formally, we have a signal space $\mathcal{S}$, alternatives $\mathcal{A} = [n]$, and 
%valuations $v_i: \mathcal{S} \rightarrow \reals^+$, where for every agent $i$ and signal profile $\profile$, the value of agent $i$ for winning the item is $v_i(\profile)$, otherwise her value is $0$.
%
% \vspace{1ex}
% \noindent{\bf Reduction to public projects.} Given any instance $(n, \mathcal{S},\mathcal{A},\vprofile)$ in the single-item auctions setting (i.e., $\mathcal{A}=[n]$), 


Given a single-item auction instance $(n, \mathcal{S},\mathcal{A},\vprofile)$, we define a public projects instance $(n,\mathcal{S},\vprofile',n, 1)$ with $n$ agents,  $m=n$ projects and $k=1$ (i.e., a single project should be chosen), where the valuation function $v'_i: [n]\times\mathcal{S} \rightarrow \reals^+$ is defined as
\[
    v'_i(j; \profile)= \begin{cases}
                          v_i(\profile) &\text{ if } j = i,\\
                          0 &\text{ otherwise }
                        \end{cases}
\]
%\michal{Would be good to add here something about the reduction, beyond the construction.} 
That is, in the reduced instance, for every $j=1,\ldots,n$, we have a project $j$ associated with the outcome ``$j$ wins the item'', and only agent $j$ has non-zero value for this project. 
Thus, the social welfare of allocating a project $j$ (possibly, at random) in the public projects setting equals the social welfare of allocating the item to bidder $j$ in the corresponding auction setting, and the reduction is approximation preserving. 
As a corollary, the impossibility results for auction settings from~\citep{EFFG18} carry over to  public project settings. 

%Similarly, we can define a reduction from any single-dimensional setting (e.g., multi-unit auctions) to public projects, implying that the public projects setting is (at least) as hard as any single-dimensional setting. 



%\divya{add that the allocation preserves welfare and we get a corollary that the impossibliites from auctions translate here.}
%\michal{I find this last paragraph a bit unclear. It's hard to understand that we're reducing $k$ identical items to the choice of $k$ public projects. I'd be happy to have a more explicit statement here.}
% Therefore, we see that all lower bound results from auctions with IDV hold in the public projects setting with IDV.
%\michal{Also: do we want to add that this is an approximation-preserving reduction?}

%\michal{I think what we should do is the following: 
% (1) present the reduction and explain the statement and the fact that it's approximation preserving.
% (2) state the results for auctions from Eden 2018 and say that these impossibilities carry over to public projects by the reduction. 
% (3) give the examples for completeness, in the terminology of public projects.}


\vspace{1ex}
\noindent{\bf Known lower bounds for single-item auctions.} 
%By the above reduction, Known impossibility results for single-item auctions in the IDV setting imply impossibility results for public projects in the IDV setting. 
The following example shows that in the absence of single-crossing, no deterministic mechanism can obtain any approximation guarantee for the optimal social welfare, even under SOS valuations.

%\avi{I copied these examples almost verbatim from \cite{EFFGK19}, we should reword them slightly.}

\begin{example}[No bound for deterministic mechanisms \citep{EFFG18}]
    \label{eg:impossiblity-deterministic}
    Consider a single-item auction with two agents. %ftwo projects $P_A$ and $P_B$. As per the reduction from auctions shown above, $P_i$ may be viewed as the project: ``player $i$ wins", for $i\in\{A,B\}$. %Thus, $v_i(P_j;\cdot)\equiv 0$ whenever $i\neq j$.
    Only agent $1$ has a signal, denoted by $s_1\in \{0,1\}$. The valuations of the agents for winning the item are
    \begin{align*}
        v_1(s_1) &= 1 + s_1, &
        v_2(s_1) &=H\cdot s_1,
    \end{align*}
    where $H$ is arbitrarily large. If the item is not allocated to agent $1$ when $s_1 = 0$, then the approximation ratio is infinite. On the other hand, if the item is allocated to agent $1$ when $s_1 = 0$, then by weak monotonicity, agent $1$ must also be allocated at $s_1=1$, leading to a $2/H$ fraction of the maximal social welfare.
\end{example}

One can easily verify that in Example~\ref{eg:impossiblity-deterministic}, no randomized mechanism can give better than $1/2$-approximation.

% \begin{example}[No bound for deterministic mechanisms \citep{EFFG18}]
%     \label{eg:impossiblity-deterministic}
%     There are two players, $A$ and $B$, and two projects $P_A$ and $P_B$. As per the reduction from auctions shown above, $P_i$ may be viewed as the project: ``player $i$ wins", for $i\in\{A,B\}$. %Thus, $v_i(P_j;\cdot)\equiv 0$ whenever $i\neq j$.
%     Only player $A$ has a signal $s_A\in \{0,1\}$. The valuations are
%     \begin{align*}
%         v_A(P_A;s_A) &= 1 + s_A&  v_B(P_A;s_A) &=0 \\ 
%         v_A(P_B;s_A) &= 0&  v_B(P_B;s_A) &=H\cdot s_A,
%     \end{align*}
%     where $H$ is arbitrarily large. If $P_A$ is not chosen when $s_A = 0$, then the approximation ratio is infinite. On the other hand, if $P_A$ is chosen when $s_A = 0$, then by weak monotonicity, $P_A$ must also be chosen at $s_A=1$, yielding a $2/H$ fraction of the maximal social welfare.
% \end{example}


% \michal{This claim needs an explanation. Also add that $1/2$ is what one would get by choosing a random project.}
% % for Example~\ref{eg:impossiblity-deterministic}.
% Notice that this example consists of SOS valuations. % (as the valuations are linear in the signals). 
% In fact, this $1/2$ approximation is the strongest lower bound known for auctions with SOS valuations.\divya{make this clear} \michal{I didn't understand this last sentence.} 
% The proof is quite simple%
% %
% \footnote{To get an $\alpha$ approximation, at $s_A=0$, $P_A$ must be chosen with probability at least $\alpha$. By weak monotonicity, $P_A$ must also be chosen with probability at least $\alpha$ at $s_A=1$. Therefore, $P_B$ can be chosen with probability at most $1-\alpha$ at $s_A=1$. This limits the approximation ratio to be at most $1/2$.}
% %
% and it inspires the more involved proof of our lower bound for public projects presented in Theorem~\ref{thm:lower-bound} below. 

Beyond SOS valuations, no non-trivial approximation can be obtained by any truthful mechanism, as the next example shows.
\begin{example}[Lower bound of $n$ for randomized mechanisms without SOS \citep{EFFG18}]
    \label{eg:impossiblity-without-exclusion}
    Consider a single-item auction with $n$ agents. % and $n$ projects $P_1, \ldots,P_n$. As in the previous example $P_i$ can be viewed as the project ``agent $i$ wins'', for all $i\in [n]$, and $v_i(P_j;\cdot)\equiv 0$ whenever $i\neq j$. 
    For every agent $i$, $s_i\in \{0,1\}$, and the valuation of agent $i$
 for winning the item is
 \[
        v_i( \profile)=\prod_{j\neq i} s_j + \varepsilon\cdot s_i. %\quad \mbox{for } \varepsilon \to 0; 
    \]
    That is, agent $i$'s value for the item is non-negligible if and only if the signals $\sminus$ are $(1,\dots,1)$. When all signals are $1$, let $i$ be the agent who is allocated the item with probability at most $1/n$ (there must be such an agent in any feasible outcome). By weak monotonicity, at $\profile'=(\vec 1_{-i}, 0_i)$ the probability that agent $i$ is allocated the item is also at most $1/n$. Therefore, the welfare obtained is at most $\frac{1}{n}+\epsilon\cdot(n-1)$ at signal profile $\profile'$, while the optimal welfare is $1$, thus giving a factor-$n$ gap when $\varepsilon \to 0$.
\end{example}
%By the reduction, these examples also imply impossibility results for the public projects setting (in the absence of additional conditions).
% \begin{example}[$n$ lower bound for randomized mechanisms without SOS \citep{EFFG18}]
%     \label{eg:impossiblity-without-exclusion}
%     There are $n$ agents $1,\ldots,n$ and $n$ projects $P_1, \ldots,P_n$. As in the previous example $P_i$ can be viewed as the project ``agent $i$ wins'', for all $i\in [n]$, and $v_i(P_j;\cdot)\equiv 0$ whenever $i\neq j$. For every agent $i$, $s_i\in \{0,1\}$, and 
%     \[
%         v_i(P_i; \profile)=\prod_{j\neq i} s_j + \varepsilon\cdot s_i \quad \mbox{for } \varepsilon \to 0; 
%     \]
%     that is, agent $i$'s value is non-negligible if and only if the signals $\sminus$ is $(1,\dots,1)$. When all signals are $1$, let $P_i$ be a project which is chosen with probability at most $1/n$ (there must be such a project in any feasible outcome). By weak monotonicity, at $\profile'=(\vec 1_{-i}, 0_i)$ the probability that project $P_i$ is chosen is also at most $1/n$. Therefore, the welfare obtained is at most $\frac{1}{n}+\epsilon\cdot(n-1)$ at signal profile $\profile'$, while the optimal welfare is $1$, thus giving a factor $n$ gap.
% \end{example}

%%%%%%%%%%%%%%%%%%%%%%% SECTION: IMPOSSIBILITY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\subsection{SOS to the Rescue?}
\label{sec:impossibility-result}

%   In this section we see that there is an inherent challenge in the public projects with interdependent value setting. In the combinatorial auctions setting with IDV, for any valuations that are separable SOS, we can get a 1/4-approximation~\cite{EFFGK19} to the optimal social welfare with a {universally} truthful mechanism. However, in the public projects setting we see that no {universally} truthful mechanism can guarantee more than a $1/m$-approximation even when the valuations are separable SOS. 
%   That is, without strong single-crossing, we cannot do any better than picking a project at random. The following example is inspired by Example \ref{eg:impossiblity-deterministic}.
   
      In this section we show that public projects with interdependent values impose a unique challenge that does not arise in auction settings. 
   In combinatorial auctions with interdependent values, the SOS property (combined with separability) comes to our rescue; in particular, there exists a universally truthful mechanism that gives $1/4$-approximation to the optimal welfare for any instance with separable SOS valuations~\citep{EFFGK19}. 
   In stark contrast, the following theorem shows that in public projects, no {universally} truthful mechanism guarantees more than a $1/m$-approximation, even for separable SOS valuations. 
   
% \michal{Instead of presenting the example first and the theorem next, I would just state the theorem, and present the instance as part of the proof. Just start the proof by "Consider the public projects instance, inspired by Example \ref{eg:impossiblity-deterministic}.
% }
         

 
   

%-------------------- OMITTED STUFF ----------------------------%
\Omit{
We will first prove some claims that will help us to get the lower bound result. 

\begin{corollary}
Let $M$ be any randomized mechanism, where an output of $M$ is a distribution over outcomes in $\mathcal{A}$, and we denote the value of a randomised allocation $a$ by $v_i(a,\profile) = E_{\alpha \sim a}[v_i(\alpha,\profile)]$.

A randomized mechanism $M$ is ex-post universally truthful only if  it satisfies weak monotonicity with respect to the expected valuation. 
\end{corollary}


\dnote{DM: We will have w-mon/single-crossing is necessary even for truthful in expectation.}
\begin{proof}
Since any universally truthful mechanism is a distribution over deterministic truthful mechanisms and by Theorem~\ref{} we see that weak monotonicity holds for each and every truthful mechanism, and hence it holds in expectation.
\end{proof}
}
%-----------------------------------------------------------------%

%\dnote{Example~\ref{eg:impossiblity-deterministic} also provides an impossibility beyond deterministic mechanisms. No randomized mechanism can do better than a $1/2$ approximation, i.e, allocating the item at random. This is because, to obtain at least a $1/2$-approximation, buyer $A$ must be allocated the item with probability at least $1/2$ at $s_A = 0$. By weak monotonicity, at $s_A =1$, buyer $A$ must still be allocated with probability $\ge 1/2$. That is, buyer $B$ only gets the item with probability at most $1/2$ at $s_A =1$, and hence the welfare achieved is at most a $1/2$ factor of the optimal welfare.  This inspires the more involved proof of our lower bound for public projects presented in Theorem~\ref{thm:lower-bound} below.}

\begin{theorem}\label{thm:lower-bound}
There exist linear valuation functions for which no ex-post IC-IR mechanism can perform better than allocating a project at random, i.e., we cannot get better than a $1/m$-approximation to the optimal social welfare.
\end{theorem}

\begin{proof}

Consider the following public projects instance, inspired by Example~\ref{eg:impossiblity-deterministic}.
   \begin{example}\label{eg:lower-bound-1/n}
    Consider $n$ agents, $m = n+1$ projects labelled $\{0 , 1, 2,\ldots, n\}$, and each agent $i\in [n]$ has a private signal $s_i \in \{0,1\}$ (using the convention that $s_{n+1} = s_1$). For any agent $i\in [n]$ and signals $\profile$, let $v_{i}(j; \profile)$ denote the value of agent $i$ for project $j$ under signals $\profile$. We define
    \[
    v_i (j; \profile) =
        \begin{cases}
        \varepsilon s_i + 1 & \text{ for }j =0,\\
        \frac{\varepsilon}{i+1} s_i + H^i\cdot s_{i+1} & \text{ for } j = i, \\
        \frac{\varepsilon}{j+1} s_i & \text{ otherwise}
        \end{cases}
    \]
    where $H$ is an arbitrarily large number.
   \end{example}
Recall that for a mechanism $(f,p)$ to be an $\alpha$-approximation (in the worst case) the (expected) welfare at each $\profile\in \{0,1\}^n$ needs to be at least an $\alpha$ factor of the optimal social welfare at $\profile$.
For $\profile = (0,0,\ldots, 0)$, project $0$ is optimal and the only outcome with positive welfare, hence any $\alpha$-approximation should allocate project $0$ with probability at least $\alpha$. For  $\profile = (1,1,\ldots,1)$ allocating project $n$ is optimal, and the welfare for any project other than $n$ is at most a $1/H$ factor of the optimal. For $\ell\le n-1$, $\profile = (0,1^{\ell},0^{n-\ell-1})$ allocating project $\ell$ is optimal, and the welfare for any project other than $\ell$ is at most a $1/H$ factor of the optimal. Hence when $\profile = (0,1^\ell,0^{n-\ell-1})$ (resp. $\profile = (1,1,\ldots,1)$), any $\alpha$-approximation should allocate project $\ell$ (resp. $n$) with probability at least $\alpha$. %In fact, for any $\profile$ where $s_\ell = 1$ and $s_j = 0$ for all $j>\ell$, we need to allocate project $\ell$ with probability at least $\alpha$.

%However, by Lemma~\ref{lem:wmon-necessary} we know that any ex post IC-IR  mechanism $(f,p)$ needs to satisfy generalized W-Mon \avi{gen.-W-Mon has not been defined yet} (or, equivalently, by Theorem~\ref{thm:linear-characterization} $\vprofile$ satisfies $f$-single-crossing).
However, by Theorem~\ref{thm:linear-characterization}, for any truthfully implementable $f$ it holds that  $\vprofile$ satisfies $f$-single-crossing, since the valuations are linear (and hence decomposable).
Observe that, for all $i$ and $\sminus$ the slope $\pdif{v_i}{s_i}(j; \profile)$ is \emph{decreasing} in $j$. That is, for all $j_1 < j_2$ we have $v_{i} (j_1; s_i',\sminus) - v_{i} (j_1; \profile)> v_{i} (j_2; s_i',\sminus) - v_{i} (j_2; \profile)$, for $s_i' > s_i$. Thus, by $f$-single-crossing any truthfully implementable social choice function $f$ cannot both allocate $j_1$ at $\profile$ and $j_2 $ at $(s_i',\sminus)$ (it can only do one or the other). 

This implies, if $f$ allocates $\ell$ at $(0,1^\ell,0^{n-\ell-1})$ for $0\le \ell< n$, then at $(0,1^{\ell'},0^{n-\ell'-1})$ (resp. $(1,\ldots,1)$) it cannot allocate project $\ell'\neq\ell$ (resp. $n$). Recall, however, that for every project $0\le \ell< n$, project $\ell$ must be allocated with probability at least $\alpha$ at the signal $(0,1^\ell,0^{n-\ell-1})$, and by the previous claim these events must be disjoint. Therefore, with probability at least $n \cdot \alpha$ the social choice function $f$ allocates some project other than $n$ at the signal $(1,\ldots,1)$. Since the probability that project $n$ is allocated at $(1,\ldots,1)$ must be at least $\alpha$, this implies that $1-n\cdot\alpha \geq \alpha$. Therefore, $\alpha \leq 1/(n+1)$, and hence proving the required lower bound.

The last example shows that, in the absence of strong single-crossing, we cannot do any better than picking a project at random. Unlike auction settings, SOS does not come to our rescue.
%We prove by induction that for $0<\ell\leq n$ the probability that a project $\ell'<\ell$ is chosen at $(0,1^{\ell'},0^{n-\ell'-1})$ is at least $\ell \cdot \alpha$. For the base case, $\ell = 1$, notice that by W-Mon the probability that project 0 is chosen at $(0,1,0^{n-2})$ must be at least the probability it is chosen at $\vec 0$. For the step, assume that
% Thus, with probability at least $n \alpha$ we cannot allocate project $n$ at $(1,\ldots,1)$, because in all instances where we allocate project $0\leq \ell < n$ at $(0,1^\ell,0^{n-\ell-1})$ we cannot allocate project $n$ at $(1,\ldots,1)$ and the cases for distinct values of $\ell$ are mutually exclusive (since we can't switch from $\ell$ to $\ell+1$). Recall that with probability at least $\alpha$ we allocate project $n$ at $(1,\ldots,1)$. So we need $(n+1)\alpha \le 1$, i.e., $\alpha \le 1/(n+1)$, and hence proving the required lower bound.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%% SECTION: APPROX WITH EXCLUSION %%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Exclusion Allows Approximation} 
\label{sub:exclusion-to-rescue}
% with Capacities}

%\inbal{from meeting: need to show reduction from $k>1$ and even any social choice func, to $k=1$, for the approximation results to hold}
   
% In the public projects setting, the above impossibility result shows that even when valuations are separable SOS we cannot do better than randomly allocating a project. 
% \michal{I added a concluding sentence in the end of the last subsection, and now I think we can remove the first sentence here, and start this subsection with what's coming next:}

% In this section, we modify the model of public projects to circumvent this barrier.
% We identify ``excludability'' as a key property that enabled the universally truthful $1/4$-approximation \cite{EFFGK19} in the auctions setting . The mechanism in~\cite{EFFGK19} selects a set of agents to be entirely excluded from the allocation. This is a crucial step, as it allows to extract truthful reports in the absence of single crossing.
% %requires the capability to completely exclude a subset of the agents from the allocation.
% However, this is fundamentally impossible in the public projects setting. To apply an approach similar to \cite{EFFGK19}, we consider a modified setting where we can exclude some agents from using projects. This allows us to obtain a $1/4$-approximation to the social welfare with a universally truthful mechanism. 

A key property that enables a universally truthful mechanism with constant-factor approximation in the auctions setting is {\em excludability}. 
Indeed, the mechanism in \citep{EFFGK19} entirely excludes a chosen set of agents from being allocated. 
This is a known tool for truthfulness~\cite{GoldbergHW01,EFFGK19}: the excluded agents have nothing to lose, and thus would report their valuations (or signals, in IDV settings) truthfully. 
Then, it only remains to show that by excluding agents cleverly enough, the loss in welfare is limited. 
Unfortunately, the situation with public projects is different.
In contrast to auctions, where goods are allocated to individual agents, pure public goods are non-excludable by definition.
Apparently, this challenge leads to the impossibility result cast in Theorem~\ref{thm:lower-bound}.
%
To alleviate this barrier, we turn to a variant of public goods that allows for exclusion. 

%In this setting, we again have $n$ agents and $m$ projects and we want to build at most $k$ projects. However, we can choose which subset of agents would get to use the projects we allocate. 

%Note that, wlog allocations that maximize welfare do not exclude any agents, that is, all agents get to use the projects. 

%\subsection{Excludability}
%\label{sec:club-prelims}
%\inbal{consider pushing this to section 4}

\vspace{1ex}
\noindent{\bf Excludable public projects.} %The setting of excludable public projects is also known in the literature as ``club goods''.  % AVI: SEE IF CAN ADD A MORE RECENT AND RELEVANT CITE.
We consider the setting of excludable public projects~\citep{DR99a, DR99b} (also known as ``club goods"). In this setting, for each project $j$ chosen by the mechanism, the mechanism is allowed to exclude a set of agents $E_j \subseteq [n]$ from using it. 
That is, agents in $E_j$ obtain no value from project $j$. %, while the remaining agents $i\in[n]\setminus E_j$ obtain a value of $v_i(j; \vec s)$ from project $j$.
%That is, the value agent $i$ obtains for a set of projects $J\subseteq [m]$ after exclusion is equal to her value for the set of projects from which she is not excluded, i.e., $J'=\{j\in J \mid i\notin E_j\}$.% had there been no exclusion.
%\divya{formalize with $(n,S,A,v)$ notation.} 
%
In fact, our results hold even with respect to a more restricted class of mechanisms where $E_j = E_{j'}$ for every $j,j'\in[m]$; i.e., the set of excluded agents is identical for all projects.

Formally, an instance of \emph{globally excludable public projects} is defined by the tuple $(n, \mathcal{S},m,\vprofile, k)$, where a feasible outcome is given by a set $J \subseteq [m]$ of size at most $k$, along with a set $E\subseteq[n]$ of excluded agents. Slightly overloading notation, the valuation $v_i$ is defined as $v_i(J,E;\profile) = v_i(J;\profile)$  for $i\notin E$ and zero otherwise.

% Observe that exclusion compromises on welfare, since any excluded agent $i\in E$ can no longer contribute to the social welfare. However, we immediately see that exclusion can be useful to extract truthful signals partially.
% For example, consider any mechanism that always excludes a subset of agents $A$. 
% We can extract truthful signals from agents in $A$ since they have no incentive to lie (i.e., they get nothing no matter what they say). It is important to note that this implication only holds when we impose global exclusion on the mechanism, i.e., the agents in $A$ must be excluded from all projects. Otherwise, a partially excluded agent still gets non-zero value when projects she is not excluded from get allocated, and therefore would indeed have an incentive to report her signal untruthfully.

Global exclusion is useful for the design of truthful mechanisms. Indeed, as in the case of auctions, the excluded agents gain no benefit no matter what they report, and would therefore lose nothing from reporting their signals truthfully.

Notably, this is not the case for ``local exclusion", namely, where every project has a different set of excluded agents.
Indeed, an agent who is excluded from some project $j$ may still wish to misreport her signal in order to affect the allocation of a different project she is not excluded from.
Interestingly, even if agents have independent signals for different projects (this setting is beyond the one we consider here), an agent who is excluded from some project $j$ may still have incentive to lie about her signal for project $j$, since it may affect the allocation of different projects (see Appendix \ref{app:local-exclusion} for an example). 
%\michal{Add an example}\divya{Please check}\avi{The example is correct, but why do we want a multi-signal example? Why not just have $s_1$ and $s_2$ in the valuations?}\divya{because this is a stronger statement, it might seem obvious that if $s_1$ affects all the projects then agent one can misreport $s_1$ to influence the project that she is not excluded from}

% \begin{definition}[$A$-exclusion mechanism]
% Let $A\subseteq [n]$ be any subset of agents. Given any valuation functions $\vec{v}(\cdot)$, we say that a mechanism/social choice function $F$ is an $A$-exclusion mechanism if for all signal profile $\profile$, $F(\profile)$ allocates nothing for all agents $i\in A$. 
% \end{definition}

% \vspace{1ex}
% \noindent{\bf Reduction.} %\avi{Actually the reduction only works when we have ( exclusion (unless we do the general reduction where each possible outcome is reduced to a distinct project rather than each $k$ tuple of project)}
% We can reduce any instance of public projects with $k>1$ to an instance of public projects with $k=1$. Therefore, any approximation guarantee for instances with $k=1$ provides a general approximation for all $k\geq 1$ (at the cost of a factor $k$ exponential blowup in the size of the instance). Given an instance of public projects $(n, \mathcal{S},m,\vprofile, k)$ with $n$ agents, we define the following public projects instance $(n, \mathcal{S},m',\vprofile', 1)$, where each project in $[m']$ represents a $k$-tuple of projects in $[m]$, i.e., $m' = \binom{m}{k}$,
% and the valuation function $v_i': m'\times \mathcal{S}\to \reals^+$ is defined as
% \[
%     v_i'(J;\profile)=v_i(\{j_1,\ldots, j_k\}; \profile)
% \]
% where $J\in [m']$ corresponds to the set of $k$ projects $\{j_1,\ldots,j_k\} \subset [m]$. Note that this reduction also applies to IDV public projects settings with \emph{global exclusion}, as in such instances each excluded agent is excluded from all projects. Therefore, we can simply keep the set of excluded agents the same in the reduced instance, and these agents receive a value of zero as they did in the original instance.

Clearly, exclusion might harm welfare, as the excluded agents contribute nothing to the social welfare. 
Our main positive result is that the universally-truthful mechanism devised in \citep{EFFGK19} can be adapted to excludable public goods, and the same $1/4$-approximation to the optimal social welfare applies.

%\michal{We start with an observation showing that... (please complete). Please also rewrite the observation in a clearer way.}
We first observe that it is without loss of generality (computational considerations aside) to restrict attention to the case where a single project should be chosen (i.e., $k=1$). 
%any instance of globally excludable public projects setting can be reduced to an instance of globally excludable public projects with $k=1$. As discussed previously, without exclusion, any social choice setting can be reduced to a public projects setting with $k=1$. Further, since the exclusion is ``global'' it naturally translates in the reduction.} 
Indeed, given an instance $(n,\mathcal{S},m,\vprofile,k)$ where $k$ projects should be chosen, one can consider an instance $(n,\mathcal{S},{m \choose k},\vprofile',1)$, where every $k$-project set in the original instance is a ``meta-project" in the new instance, and $v'_i(J,E;\profile) = v_i(J,E;\profile)$.


%\begin{observation}
% Given any instance, $(n,\mathcal{S},m,\vprofile,k)$, of globally excludable public projects with $k >1$ we can reduce it to an instance, $(n,\mathcal{S},{m \choose k},\vprofile',1)$, of globally excludable public projects with \emph{one project}, where $v'_i(J,E;\profile) = v_i(J,E;\profile)$ by considering a set of $k$ projects in the former as a ``meta project'' in the reduced instance.
%\end{observation}

\vspace{1ex}
\noindent{\bf Approximation.}
%\divya{[segue with extending this intuition to get a mechanism that is truthful for all agents.]}
We consider the \textsf{Random-Sampling-VCG} mechanism, introduced in~\cite{EFFGK19} for combinatorial auctions, adapted to excludable public projects as described below. 

For any setting with separable valuations, \textsf{Random-Sampling-VCG} is a universally truthful mechanism. This property arises from the fact that globally excluded agents have no incentive to lie about their signals as they get nothing in any possible outcome. Further, if the valuations are SOS, then using the key lemma (Lemma \ref{lem:key-lemma}), we get a $1/4$-approximation to the optimal welfare.

 \begin{theorem}\label{thm:4-approx}
 There is an ex-post IC-IR mechanism that guarantees a $1/4$-approximation for the optimal social welfare under the setting of excludable public projects with separable SOS valuations.
 \end{theorem}
 
We focus on globally excludable settings, as global exclusion is all that is required for this mechanism. Moreover, due to the reduction shown above, we may restrict our attention to settings with $k=1$.
We start by considering the following class of mechanisms, similar to the VCG-inspired mechanisms from ~\cite{EFFGK19}.

\begin{definition}[\textsf{$A$-exclusion-VCG}]
 Given any valuations $\vprofile$, and a subset of agents $A$, we define the \textsf{$A$-exclusion-VCG} mechanism as follows:
\begin{enumerate}
    \item All agents report some signals $\tilde{s_i}\in S_i$.
    \item For agents $i\notin A$, define $w_i(a;\tilde{s_i},\tilde{\mathbf{s}}_{A}) = v_i(a;\tilde{s}_i,\tilde{\mathbf{s}}_{A},\vec 0_{A^c\setminus \{i\}})$ for all projects $a$.
    \item Allocate $a^*\in \argmax_a \sum_{i\notin A} w_i(a;\tilde{s}_i,\tilde{\mathbf{s}}_{A})$.
    \item Compute generalized VCG prices for all $i\notin A$, 
        \[
            p_i(\tilde{\mathbf{s}}) = \left(g_{-i}(a^*;\tilde{\mathbf{s}}_{-i}) - g_{-i}(a^*;\tilde{\mathbf{s}}_{A},\vec 0_{A^c\setminus\{i\}})\right) - \sum_{i'\notin A\cup\{i\}} w_{i'}(a^*;\tilde{s}_{i'},\tilde{\mathbf{s}}_{A}) + \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;\tilde{s}_{i'},\tilde{\mathbf{s}}_{A})
        \]
\end{enumerate}
\end{definition}

\begin{lemma}\label{lem:A-exclusion-truthful}
The \textsf{$A$-exclusion-VCG} mechanism is truthful when the valuations are separable SOS\footnote{We actually do not need the full SOS property, we only need $v_i(a;\profile) = h_i(a;s_i) + g_{-i}(a;\sminus)$.}. 
\end{lemma}

\begin{proof}[Proof. {[Following \cite{EFFGK19}, Theorem 5.1]}]
% \dnote{DM: easiest way to show this is to define the generalized vcg prizes and show that because of separability the dependence on $s_i$ cancels out. We could also show it is W-Mon for separable functions (but since W-Mon isn't sufficient in general, maybe we shouldn't go that way).} 
% \avi{should we change the word "outcomes" to "projects"?}
%
For any agent $i$ with true signal $s_i$, and fixed $\tilde{s}_{-i} = \sminus$, we show that her utility for reporting $\tilde{s}_i = s_i$ is at least her utility for reporting $\tilde{s}_i = s'_i$ for all $s'_i\neq s_i$.

Clearly, for any $i\in A$, the utility of $i$ is $0$ (with no allocation and $0$ payment) for any reported signal. Hence truthfulness trivially follows.
Let $f(\profile)$ be the output of the $A$-exclusion mechanism for any reported signals $\tilde{\mathbf{s}} = \profile$. For any agent $i\notin A$, observe that the price $p_i(\tilde{\mathbf{s}})$ does not depend on $\tilde{s_i}$. For separable SOS valuations, with $v_i(a,\profile)= h_i(a;s_i) + g_{-i}(a;\sminus)$ we have $w_{i}(a;\tilde{s}_i,\tilde{\mathbf{s}}_A) = h_i(a; \tilde{s}_i) + g_{-i}(a;\tilde{\mathbf{s}}_A,\vec 0_{A^c\setminus \{i\}})$. Thus we see that for all $\tilde{s}_i$ and $\tilde{\mathbf{s}}_{-i} = \sminus$ and $\hat a=f(\tilde{s}_i,\sminus)$

\begin{align*}
    p_i(\tilde{s}_i,\sminus) &= \left(g_{-i}(\hat a;\sminus) - g_{-i}(\hat a;{\profile}_{A},\vec 0_{A^c\setminus\{i\}})\right) - \sum_{i'\notin A\cup\{i\}} w_{i'}(\hat a;{s}_{i'},{\profile}_{A}) + \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;{s}_{i'},{\profile}_{A}) \\
    &= \left(g_{-i}(\hat a;\sminus) - g_{-i}(\hat a;{\profile}_{A},\vec 0_{A^c\setminus\{i\}})\right) + w_{i}(\hat a;{s}_{i},{\profile}_{A}) - \sum_{i'\notin A} w_{i'}(\hat a;{s}_{i'},{\profile}_{A}) + \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;{s}_{i'},{\profile}_{A}) \\
    &= v_i(\hat a;\profile) - \sum_{i'\notin A} w_{i'}(\hat a;{s}_{i'},{\profile}_{A}) + \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;{s}_{i'},{\profile}_{A})
\end{align*}



% We first observe that, for any \emph{separable} valuation function $v_i$, the payment $p_i(\profile)$ only depends on the allocation $a^* = f(\profile)$ and $\sminus$. This is simply because $v_i(a^*;\profile) = h_i(a^*;s_i) + g_{-i}(a^*;\sminus)$ and $w_{i}(a^*;s_i,\profile_A) = h_i(a^*;s_i) + g_{-i}(a^*;\profile_{A},0_{A^c\setminus\{i\}})$, and thus we have 
% \begin{align*}
%     p_i(\profile) &= v_i(a^*;\profile) - \sum_{i'\notin A} w_{i'}(a^*;\tilde{s}_{i'},\tilde{s}_{A}) + \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;\tilde{s}_{i'},\tilde{s}_{A}) \\
%     &= \left(g_{-i}(a^*;\sminus) - g_{-i}(a^*;\profile_{A},0_{A^c\setminus\{i\}})\right) - \sum_{i'\notin A\cup\{i\}} w_{i'}(a^*;\tilde{s}_{i'},\tilde{s}_{A}) + \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;\tilde{s}_{i'},\tilde{s}_{A}
% \end{align*}



Hence we have that the utility of agent $i$ with true signal $s_i$ and reported signal $\tilde{s}_i$ is, 
\[
  v_i(f(\tilde{s}_i,\sminus);\profile) - p_i(\tilde{s}_i,\sminus) =   \sum_{i'\notin A} w_{i'}(\hat a;{s}_{i'},{\profile}_{A}) - \left( \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;{s}_{i'},{\profile}_{A})\right)
\]

Note that, the first term is maximized at $\hat a = f(\profile)$ by definition of our social choice function. Thus, the utility of agent $i$ for $\tilde{s}_i = s_i$ is maximal.

Moreover, we note that the utility at $\tilde{s}_i = s_i$ is non-negative. This is because the first term is larger than the second term due to reason similar to VCG.
% For each agent $i$, signal profile $\profile$, and $s'_i$. Let $a^* = f(\profile)$ and $a' = f(s'_i\sminus)$. Therefore, the utility of agent $i$ for reporting her true signal $s_i$ is,
% \[
%   v_i(f(\profile);\profile) - p_i(\profile) =   \sum_{i'\notin A} w_{i'}(a^*;{s}_{i'},{s}_{A}) - \left( \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;{s}_{i'},{s}_{A})\right)
% \]
% and the utility of agent $i$ for misreporting her signal as $s'_i$ is,
% \[
%   v_i(f(s'_i,\sminus);\profile) - p_i(s'_i,\sminus) =   \sum_{i'\notin A} w_{i'}(a';{s}_{i'},{s}_{A}) - \left( \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;{s}_{i'},{s}_{A})\right)
% \]
% Next we observe that the allocation $f(\profile) = a^*$ is a utility maximizer \footnote{Such mechanisms are termed pseudo-efficient in \citet{CE02}, and shown to be ex-post IR and ex-post IC.} for all agents $i$. This is because for all agents $i \not in$, 
%
% \[
%     a^* \in \argmax_{a} \{v_i(a;\profile) - p_i(\profile)\} = \left(\argmax_{a} \{\sum_{i'\notin A} w_{i'}(a^*;\tilde{s}_{i'},\tilde{s}_{A})\}\right) - \left( \max_{a} \sum_{i' \notin A\cup\{i\}}w_{i'}(a;\tilde{s}_{i'},\tilde{s}_{A}) \right).
% \]
\end{proof}

The \textsf{$A$-exclusion-VCG} mechanism assumes an arbitrary set $A$ of excluded agents. This is used as a subroutine in the mechanism for which we obtain our approximation result, defined as follows.

\begin{definition}[\textsf{Random-Sampling-VCG}]\label{def:random-sampling-vcg}
Randomly sample a subset of agents $A\subseteq [n]$ uniformly at random. Then run the $A$-exclusion-VCG mechanism.
\end{definition}

By Lemma~\ref{lem:A-exclusion-truthful}, for every fixed $A\subseteq [n]$ the \textsf{$A$-exclusion-VCG} mechanism is truthful, therefore we obtain the following corollary.

\begin{corollary}~\label{cor:univ-truthful}
\textsf{Random-Sampling-VCG} is a universally truthful mechanism when the valuations are separable SOS.
\end{corollary}
%  \divya{add discussion about local exclusion is not enough for truthfulness?}
% \avi{I don't remember this discussion... How can local exclusion not be enough for truthfulness when global exclusion is a subcase of local exclusion? Do we simply want to say that if an agent is excluded from some but not all of the projects it still has an incentive to lie?}

%We then invoke the Key Lemma from~\cite{EFFGK19}, to show that when we randomly sample $A$, we get a $1/4$-approximation to the optimal welfare for SOS valuations.

The final component we need for the proof of the theorem is the Key Lemma (\citet{EFFGK19}).

\begin{lemma}[Key Lemma, ~\cite{EFFGK19}]\label{lem:key-lemma}
Let $v_i : {(\reals^+)}^n \rightarrow \reals^+$ be any SOS function. Let $A$ be a uniformly random subset of $[n]\setminus \{i\}$ and $B = A^c\setminus\{i\}$. Then we have for all $\profile$, 
$\E_A[v_i(s_i,\profile_A,\vec 0_B)] \ge \frac{1}{2}v_i(\profile).
$
\end{lemma}

We are now ready to prove the theorem. 

\begin{proof}[Proof of theorem~\ref{thm:4-approx}]
For every profile $\profile$, $i\in [n]$ and $a\in \mathcal{A}$, we have
 \[
     \E_A[w_i(a;s_i, \profile_A)\cdot\one_{\{i\notin A\}}] = \E[v_i(a;s_i,{\profile}_A,\vec 0_{A^c\setminus\{i\}})\mid i \notin A]\Pr[i \notin A]  \ge \frac{1}{4}v_i(a;\profile).
 \]
 
This follows from Lemma~\ref{lem:key-lemma}, because $v_i(a;\cdot)$ is an SOS function. Therefore, for any $\profile$ let $\tilde{a}$ be a welfare maximizing allocation. For every subset $A$, the social welfare of  \textsf{$A$-exclusion-VCG} is $\sum_{i\notin A} v_i(a^*;\profile) \ge \sum_{i\notin A} w_i(a^*;s_i,\profile_A)$ when $a^* \in \argmax_{a\in\mathcal{A}}\sum_{i\notin A} w_i(a;s_i,\profile_A)$.

Hence the social welfare of the \textsf{Random-Sampling-VCG} is at least

% \begin{align*}
%     \E_{A}\Big[\max_{a\in \mathcal{A}}\sum_{i\notin A} w_i(a;s_i,s_A) \Big] &\ge \E_{A}\Big[\sum_{i} w_i(\tilde{a};s_i,s_A)\cdot \one_{\{i\notin A\}}\Big] \\
%     &= \sum_{i}\E_{A}[ w_i(\tilde{a};s_i,s_A)\cdot \one_{\{i\notin A\}}] \\
%     & \ge \frac{1}{4} \sum_{i}v_i(\tilde{a};\profile).
% \end{align*}

$$
    \E_{A}\Big[\max_{a\in \mathcal{A}}\sum_{i\notin A} w_i(a;s_i,\profile_A) \Big] \ge \E_{A}\Big[\sum_{i} w_i(\tilde{a};s_i,\profile_A)\cdot \one_{\{i\notin A\}}\Big] 
    = \sum_{i}\E_{A}[ w_i(\tilde{a};s_i,\profile_A)\cdot \one_{\{i\notin A\}}] 
     \ge \frac{1}{4} \sum_{i}v_i(\tilde{a};\profile).
$$
\end{proof}



==> arXiv version/general-charac.tex <==
\section{General Characterization of Social Choice Implementability}\label{sec:general-charac}

In this section we complement our characterization results from Section~\ref{sec:linear-characterization}. In Section~\ref{sub:beyond-decompose} we define \emph{weak} $f$-single-crossing and show that it characterizes implementability for general IDV settings. In Section~\ref{sec:idv-ipv-equiv} we discuss the connections between implementability in IPV and IDV, showing in particular that weak $f$-single-crossing is analogous to C-Mon and $f$-single-crossing is analogous to W-Mon. In Section~\ref{sub:impossibility-for-non-decomposable} we identify decomposable valuations as precisely the class for which W-Mon characterizes implementability, thus mirroring convex domains in IPV settings. 

\subsection{Beyond Decomposable Valuations}
\label{sub:beyond-decompose}

For general valuations beyond decomposable, a more complex condition for characterizing implementability than $f$-single-crossing is needed. The explanation for this is as follows:
In the case of decomposable valuations~$\vprofile$, the decomposability property naturally ensures that for every $i$,  $\sminus$ and outcomes $a,b\in \Delta(A)$, either $\pdif{v_i}{s_i}(a;s_i,\sminus) \le \pdif{v_i}{s_i}(b;s_i,\sminus)$ for all $s_i \in S_i$, or $\pdif{v_i}{s_i}(a;s_i,\sminus) \ge \pdif{v_i}{s_i}(b;s_i,\sminus)$ for all $s_i \in S_i$. In other words, %for any decomposable valuation $v_i$ and fixed $\sminus$, 
the slopes $\pdif{v_i}{s_i}$ induce a global ordering of the outcomes that does not depend on $s_i$. This will not necessarily hold for general valuations and so $f$-single-crossing is ill-defined for such valuations.
%and this invokes a need for a more complex condition for characterizing implementability.
%%%%--gen-f-single-crossing-REMOVED
% We first define a natural generalization of $f$-single-crossing for general valuations, which we show to be a sufficient \michal{(but not necessarily a necessary)} condition for truthful implementability. 
% %However, this is not a necessary condition under general valuations. 
%
% \begin{definition}\label{defn:single-crossing}
%  Let $f$ be some social choice function.
%  We say that the valuations $\vprofile$ satisfy general $f$-single-crossing if for each agent $i$ and signal profile $\profile \in \mathcal S$
%  %such that $z > s_i$ and every $s' \in [s_i,z]$ 
%  it holds that:
%  \begin{align}
%     \left\langle \pdif{v_i}{s_i} (\profile), \; f(z,\sminus)  \right\rangle &\geq \left\langle \pdif{v_i}{s_i} (\profile), \; f(\profile)  \right\rangle \label{eq:single-crossing-condition1} &\forall z > s_i\\
%     \left\langle \pdif{v_i}{s_i} (\profile), \; f(z,\sminus)  \right\rangle &\leq \left\langle \pdif{v_i}{s_i} (\profile), \; f(\profile)  \right\rangle
%     & \forall z < s_i
%     \label{eq:single-crossing-condition2}
%  \end{align}
% \end{definition}
%
%
% Informally, for each signal profile $\profile$, the slope of $v_i$ at $s_i$ for the outcome $f(\profile)$ at $s_i$ \michal{you've written "at $s_i$" twice, shall we remove one of these?}
% is better than the slope for all ``previous'' outcomes $f(z,\sminus)$ for $z<s_i$. Similarly, the slope of $v_i$ at $s_i$ for a ``later'' outcomes $f(z,s_i)$ for $z> s_i$ is better than the slope for $f(\profile)$. Note that, under decomposable valutions this is exactly the same as $f$-single-crossing (Definition~\ref{defn:linear-f-single-crossing}).
% %Namely, for each signal profile $\profile$ and $z > s_i$ the ``slope'' of a ``later'' outcome $f(z,\sminus)$ at the point $\profile$ must be larger than the ``slope'' of the ``current'' outcome $f(\profile)$ at the same point.
%
% \michal{What's the significance of presenting the above definition? (in light of the fact that it is followed by the "right" definition)?}\inbal{From meeting - move to the appendix}
%
% It turns out the above condition is too strong and is not necessary for truthful implementation for general valuations. 
%%%%
We thus introduce the following definition and show it is the ``right'' generalization of $f$-single-crossing, in the sense that it is both necessary and sufficient for implementability. 

\begin{definition}\label{defn:weak-single-crossing}
 Let $f$ be a social choice function. We say that the valuations $\vprofile$ satisfy \emph{weak} $f$-single-crossing if for each agent $i$ and signal profile $\profile \in \mathcal S$, and for every $z \in S_i$ %such that $z > s_i$ 
 it holds that:
 \begin{equation}\label{eq:weak-single-crossing-condition}
    \left\langle v_i(z,\sminus) - v_i(\profile), \; f(z,\sminus)  \right\rangle \geq \int_{s_i}^{z} \left\langle \pdif{v_i}{s_i} (t, \sminus), \; f(t, \sminus)  \right\rangle dt
 \end{equation}
\end{definition}

%\inbal{Add here the intuitive explanations of the above definition -- what is it requiring? is it like convexity?}\avi{How about the following explanation?}

The above definition can be loosely viewed as follows. For $z>s_i$, the outcome $f(z,\sminus)$ must have a marginal improvement in $v_i$ --- as we increase the signal from $z$ to $s_i$ --- which is greater than the cumulative marginal improvements made by all outcomes $f(t,\sminus)$ for all $t\in[s_i,z]$. %Otherwise, for any fixed price we set for outcome $f(z,\sminus)$, this outcome cannot maximize the utility of agent $i$ for the signal profile $(z,\sminus)$ (unless it maximizes agent $i$'s utility for $\profile$ as well). Conversely, for $z<s_i$, the outcome $f(z,\sminus)$ must have a marginal improvement in $v_i$ - as we increase the signal from $z$ to $s_i$ - which is \emph{smaller} than the cumulative marginal improvements made by all outcomes $f(t,\sminus)$ for all $t\in[s_i,z]$. Otherwise, it would have been better to stick with the same outcome, i.e., $f(z,\sminus) = f(\profile)$. Moreover, notice that whenever $f(z,\sminus) = f(\profile)$, Inequality \eqref{eq:weak-single-crossing-condition} simply becomes an equality, as we can get the reversed inequality by writing Inequality \eqref{eq:weak-single-crossing-condition} while reversing the roles of $s_i$ and $z$.


\begin{proposition}[Weak $f$-single-crossing characterizes implementability]
\label{prop:single-crossing-characterization}
    For any IDV social choice setting, a mechanism is ex-post IC-IR if and only if for every $i$, $\sminus$, weak $f$-single-crossing holds, and the following payment identity and payment inequality hold:
    \begin{align}
        p_i(\profile) &= \; p_i(0,\sminus) + \int_{0}^{s_i} \left\langle v_i(t,\sminus), \pdif{f}{s_i}(t,\sminus) \right\rangle dt ; \label{eq:payments1-single-crossing} \\
        p_i(0,\sminus) &\leq  \left\langle v_i(0,\sminus), f(0,\sminus) \right\rangle. \label{eq:payments2-single-crossing}
    \end{align}
    Moreover, if we additionally require prices to be non-negative, it is sufficient to additionally have the following payment identity:
    %\begin{align}
    $
        p_i(0,\sminus) =  \left\langle v_i(0,\sminus), f(0,\sminus) \right\rangle.
    $
    %    \label{eq:payments3-single-crossing}
    %\end{align}
\end{proposition}
%PROOF MOVED TO APPENDIX
%It is not hard to see that $f$-single-crossing implies weak $f$-single-crossing, as we show in the following lemma.
It is not hard to see that, for any decomposable valuation profile $\vprofile$, $f$-single-crossing implies weak $f$-single-crossing. 
In fact, under decomposable valuations, the two notions coincide, as we show in the following lemma.

%\michal{a grammatical question regarding the following lemma and more generally throughout the paper: do we treat $\vprofile$ as a valuation profile? in which case we should say "satisfies" instead of "satisfy". I prefer to refer to it as a valuation profile throughout rather than "valuations".}

\begin{lemma}\label{lem:sc-implies-weak-sc}
    A decomposable valuation profile $\vprofile$ satisfies $f$-single-crossing if and only if $\vprofile$ satisfies \emph{weak} $f$-single-crossing.
\end{lemma}
%PROOF MOVED TO APPENDIX
%%%-gen-f-sc-REMOVED
%Therefore $f$-single-crossing is a sufficient condition, but it does not have to be necessary. %so we obtain the following corollary.
%
% \begin{corollary}\label{cor:f-sc-sufficient}
%      For every interdependent values setting, a mechanism is ex-post IC and ex-post IR if for every $i$, $\sminus$, $f$-single-crossing holds with respect to the social choice function $f$ and the payment identity and payment inequality of Proposition \ref{prop:single-crossing-characterization} hold.
% \end{corollary}
%
%%%-gen-f-sc-REMOVED
%Moreover, under decomposable valuations it is easy to see that weak $f$-single-crossing is equivalent to $f$-single-crossing. 

%\michal{Got up to here in my pass.}

\subsection{Implementability in IDV versus IPV}\label{sec:idv-ipv-equiv}

In this section we show the parallels between single-crossing-based characterizations of implementability, and classic characterizations including C-Mon and W-Mon (see Appendix~\ref{sub:prelim-IC-IPV} for the classic definitions). Our main results in this section are Corollary~\ref{cor:weakSC-equiv-to-CMON} and Corollary~\ref{cor:SC-equiv-to-WMON},
%\inbal{from our meeting: we want to say there are a lot of interesting classes of social choice functions that are not covered by finitely-many outcomes, for example 2 items.}
% \todo{This sections needs to be completely changed to cycle monotonicity}
% \noindent\textbf{Rewrite Bullet Points:}
% \begin{enumerate}
%     \item Cycle monotonicity is necessary and sufficient for (DSIC) implementability in general independent settings.
%     \item By Chung Ely we obtain that in interdependent  (EPIC) implementability holds iff cycle monotonicity holds for every fixed $i$ and $s_{-i}$.
%     No underlying distribution, values are known.
%     \item Monotonicity domains are ones where WMon is equivalent to Cycle Monotonicity, and thus WMon is a sufficient condition.
%     \item By ABHM'10, any convex domain is a monotonicity domain.
%     \item In our setting, convexity implies linearity. Therefore WMon is a sufficient condition only for valuations that are linear in the signals.
%     \item For linear valuations, WMon is equivalent to single crossing. We can show that single crossing is sufficient and necessary for implementability even for randomized mechanisms.
% \end{enumerate}
%In this section we state the necessary and sufficient conditions for a social choice function to be implementable by an ex-post truthful mechanism using the Chung-Ely~\cite{CE02} framework (see Lemma~\ref{lem:Chung-Ely}). 
and we achieve these using the Chung-Ely~\cite{CE02} framework (recall Lemma~\ref{lem:Chung-Ely} that transfers from IPV to IDV) as well as the results of~\citet{ABMH10}. See also Figure~\ref{fig:high-level-scheme} for an illustration of these connections.

We begin by defining generalizations of W-Mon and C-Mon for IDV settings.

% In interdependent settings, Incentive Compatibility is defined \emph{ex-post}, i.e., assuming all agents other than agent $i$ report their true signal, the dominant strategy of agent $i$ is to tell the truth. Therefore, a mechanism $(f,p)$ is ex-post IC if and only if for every fixed $i$ and $\sminus$ the single agent mechanism with social choice function $f(\cdot,\sminus)$ and prices $p_i(\cdot,\sminus)$ is DSIC. This intuition is formally presented in Chung and Ely \cite{CE02} as the following equivalence of DSIC vs Ex-post IC conditions.

% \divya{Let's move this to preliminaries?}
% \begin{lemma}
% The following are equivalent:
% \begin{itemize}
%     \item In the single-agent special case, the public decision rule $g:\Theta \to A$ is incentive compatible if (resp. only if) the quadruple $(A, \Theta, v, g)$ satisfies 
%     \item In the private-value special case, the public decision rule $f : \mathcal{S} \rightarrow \mathcal{A}$ is dominant strategy incentive compatible if (resp. only if) $\forall i, \forall s_{-i}$, the quadruple $(\mathcal{A}, S_i, v_i, f(s_{-i}, \cdot))$ satisfies condition $C$.
%     \item In the interdependent-value general case, the public decision rule $f : \mathcal{S} \rightarrow \mathcal{A}$ is ex post incentive compatible if (resp. only if) $\forall i, \forall s_{-i}$, the quadruple $(\mathcal{A}, S_i, v_i(\cdot,s_{-i},\cdot), f(s_{-i}, \cdot))$ satisfies condition $C$.
% \end{itemize}
% \end{lemma}

% Using this result, we may use the characterization of single agent DSIC mechanisms to fully characterize multi-agent interdependent ex-post IC mechanisms. 

% \begin{definition}[Weak Monotonicity]
%     In the single-agent special case, a public decision rule $g$ satisfies weak monotonicity with respect to the valuation function $v$, if for every 
% \end{definition}

% Let $\mathcal{S} = \times_i S_i$ denote the signal space of the agents, and $\mathcal{A}$ denote the set of outcomes, and for all $i$ let $v_i: \mathcal{A}\times \mathcal{S} \rightarrow \reals^+$ be the valuations (that is, for public projects $v_{i}(j,\profile) = v_{ij}(\profile)$ for all $j\in [m]$). Let $F: \mathcal{S} \rightarrow \mathcal{A}$ be a social choice function. Given $v_i$ we define the conditions on $F$ that are necessary and sufficient for truthful implementation.

%\inbal{Maybe change name to W-Mon-Gen?}
\begin{definition}[W-Mon Generalized to IDV]
 Given any IDV social choice setting  with valuations $\vprofile$, a social choice function $f$ satisfies weak monotonicity (W-Mon) if for any $\profile\in \mathcal{S}$, player $i$ and signal $s'_i \in S_i$, the following holds: $f(\profile)=a$ and $f(s'_i,\sminus)=b$ implies that $v_i(b;s'_i,\sminus) - v_i(b;\profile) \ge v_i(a;s'_i,\sminus) - v_i(a;\profile)$.
\end{definition}


\begin{definition}[C-Mon Generalized to IDV]
     Given any IDV social choice setting with valuations $\vprofile$, a social choice function $f$ satisfies cycle monotonicity  (C-Mon) if for any player $i$, $\sminus$, and any set of $\ell+1$ signals $s^{(1)}_i, \ldots, s^{(\ell+1)}_i \in S_i$ with $s^{(\ell+1)}_i=s^{(1)}_i$, we have that
     $
        \sum_{k=1}^{\ell} \langle v_i(s^{(k)}_i,\sminus), f(s^{(k)}_i,\sminus) - f(s^{(k+1)}_i,\sminus) \rangle \geq 0.
     $ 
\end{definition}

The definition of a convex domain $\mathcal{V}$ 
%\inbal{first time this is mentioned} 
in IPV settings translates to the following definition in IDV settings using the Chung-Ely framework.

\begin{definition} [Convex Domain for IDV]
Given any IDV social choice setting $(n,\mathcal{S},\mathcal{A},\vec v)$, for each $i$, $\sminus$, let $V_i(\sminus) = \{v_i(\profile)\in \reals^\mu \mid  s_i \in S_i\}$.
We say that the domain is convex if the closure of $V_i(\sminus)$ is convex for each $i$ and $\sminus$.
\end{definition}

%\inbal{clarify closure? say what the domain is mathematically?}

With these definitions we get the following proposition from Theorem~\ref{thm:ipv-charaterization} and Lemma~\ref{lem:Chung-Ely} (\citet{ABMH10} and~\citet{CE02}).

\begin{proposition}
[Implementability with IDV]\label{prop:IDV-implementability}
Consider an IDV social choice setting $(n,\mathcal{S}, \mathcal{A},\vec v)$ and a social choice function $f$.
\begin{enumerate}
    \item(Cycle monotonicity is necessary and sufficient) $f$ is implementable if and only if it satisfies cycle monotonicity.
    \item(Weak monotonicity is necessary) Every implementable $f$ satisfies weak monotonicity.\footnote{For an alternative proof see Appendix~\ref{apx:proofs-for-sec-3}, Lemma~\ref{lem:wmon-necessary}.}
    \item(Weak monotonicity is sometimes sufficient) Suppose that the domain is convex, then every finitely-valued $f$ that satisfies weak monotonicity is implementable.
    \end{enumerate}
\end{proposition}

Putting together Proposition~\ref{prop:single-crossing-characterization} and bullet~(1) of Proposition~\ref{prop:IDV-implementability} we immediately get the following equivalence of weak-$f$-single-crossing and C-Mon.

\begin{corollary}
    \label{cor:weakSC-equiv-to-CMON}
For any IDV social choice setting with valuation profile $\vprofile$, it holds that a social choice function $f$ satisfies cycle monotonicity (C-Mon) if and only if $\vprofile$ satisfies weak $f$-single-crossing.
\end{corollary}

%\avi{It is pretty obvious, but do we want to explain why cycle monotonicity immediately implies weak monotonicity. This connection is depicted in Figure \ref{fig:high-level-scheme} as an arrow that currently has no label. Do we want to put a label on this arrow?}

\Omit{
Weak monotonicity can be easily derived from ex-post incentive compatibility. Therefore, for any domain weak monotonicity is necessary for $f$ to be ex-post IC implementable, and it also sufficient in many natural domains.


% LEMMA + PROOF MOVED TO APPENDIX
\begin{lemma}\label{lem:wmon-necessary}
Given any valuations $\vprofile$, a social choice function $f$ is ex-post truthfully implementable only if $f$ satisfies (generalized) W-Mon.
\end{lemma}

% MAYBE MOVE TO APPENDIX?
\begin{proof}
To see why weak monotonicity follows directly from ex-post incentive compatibility, recall that a social choice function $f$ is ex-post IC implementable if there exists a price function $p:\mathcal{S} \to \reals$ such that
\[
    \langle v_i(\profile), f(\profile)\rangle - p_i(\profile) \geq
    \langle v_i(\profile), f(s_i',\sminus)\rangle - p_i(s_i',\sminus) \qquad \forall i \in [n], \; \forall \profile \in \mathcal{S}, \; \forall s'_i \in S_i.
\]
Writing the same inequality while reversing the order of $s_i$ and $s'_i$ and summing with the inequality above, we obtain
\[
    \langle v_i(s_i',\sminus), f(s_i',\sminus) - f(\profile)\rangle \geq
    \langle v_i(\profile), f(s_i',\sminus) - f(\profile) \rangle \qquad \forall i \in [n], \; \forall \profile \in \mathcal{S}, \; \forall s'_i \in S_i,
\]
which implies $f$ is weakly monotone by definition.
\end{proof}


However, weak monotonicity is not sufficient in many domains. In general IPV settings, cycle monotonicity is the right characterization for truthful implementability.
%Putting together Rochet \cite{Rochet87} and Chung \& Ely \cite{CE02}, we see that cycle monotonicity provides a general characterization in the IDV setting as well.

Even in IPV, cycle monotonicity is a property that is hard to work with, and several works have made attempts to find nicer conditions under restricted valuation domains. Notably, \citet{SY05} show that weak monotonicity is a sufficient condition for \emph{deteministic} implementability when the valuation domain is convex. This result was extended by Ashlagi et al. \cite{ABMH10} from deterministic social choice functions to \emph{finite-valued} social choice functions (i.e., the range of the social choice function is a finite set).
}


% \begin{theorem}
% Given any valuations $v_{ij}(\cdot)$, a social function $F$ is ex-post truthfully implementable if and only if $F$ satisfies cycle monotonicity.
% \end{theorem}
%\dnote{DM: This is by putting together Rochet87 and Chung-Ely}

%\todo{Check if Chung-Ely holds for randomized mechanisms/social choice functions (because Q can be any arbitrary set, so it includes randomized outcomes?)}
% \todo{Formalize proof using the following:}
% \dnote{
% \begin{enumerate}
%     \item When defining prices such that $p_i(a,s_{-i}) = - \delta_{ca}(s_{-i})$, choose $c = f(0,s_{-i})$.
%     \item In the IPV setting, the above (where $v_i \equiv 0)$ will also ensure non-negative (and ex-post IR) prices without any offset. 
%     \item For the IdV setting, adding $v_{ic}(0,s_{-i})$ is enough to make the prices non-negative and ex-post IR.
% \end{enumerate}
% }



\vspace{1ex}
\noindent {\bf Decomposable valuations as convex domains. }
By definition, $V_i(\sminus)$ is a curve in $\reals^\mu$, and a curve can be a convex domain if only if it is a straight line. Therefore, it is easy to see that \linear valuations give rise to convex domains.
%
Less obviously, any decomposable (and continuous) valuation profile gives rise to a convex domain. The reason is that much like in \linear valuations, the \emph{direction} of the tangent to the curve $V_i(\sminus)$ remains constant for all signals $s_i\in S_i$ in decomposable valuations. %However, unlike multi-linear settings the \emph{magnitude} of the corresponding vector of derivatives changes with the signal $s_i$ in decomposable valuations. Nevertheless, since the curve moves in the same direction as we increase $s_i$ (albeit perhaps with changes in ``speed''), the path it travels must be a straight line in $\reals^m$ and thus the resulting domain $D$ would be convex.
We formalize the intuition of the discussion above in the following lemma.


\begin{lemma}
\label{lem:convex-decomposable}
Suppose $S_i$ is an interval in $\reals^+$ and $v_i$ is continuous in $s_i$. 
For each $i$, $\sminus$, let $D = \{v_i(\profile) \in \reals^\mu \mid s_i \in S_i \}$ be the induced domain, then (the closure of) $D$ is convex if and only if $v_i$ is decomposable.
\end{lemma}
\begin{proof}
    Fix some agent $i$ and signals $\sminus$.
    Suppose the domain $D$ is convex. We first establish the following claim; see proof in the appendix. 
    \begin{claim}\label{clm:convex-decomposable}
        For every two signals $s$ and $s'$ in $S_i$ and every $t\in [s,s']$ there exists some $\lambda \in [0,1]$ such that $v_i(t,\sminus) = (1-\lambda) \cdot v_i(s,\sminus) + \lambda \cdot v_i(s,\sminus)$. 
    \end{claim}
    % PROOF MOVED TO APPENDIX
    
    We next show that for any signal $s \in S_i$ there exists $\lambda(s) \geq 0$ such that $v_i(s,\sminus) = (1-\lambda(s))v_i(0,\sminus) + \lambda(s) v_i(1,\sminus)$. For $s\in [0,1]$ it follows directly from the claim above. Consider $s>1$. By the claim above, there exists $\lambda'\in(0,1]$ such that 
    $
        v_i(1,\sminus) = (1 -\lambda') v_i(0,\sminus) + \lambda'v_i(s,\sminus)
    $. 
    Now by taking $\lambda(s)=1 - 1/\lambda'$ we obtain the desired equality.
    
    We conclude that $v_i$ can be written as $v_i(\profile) = \lambda(s_i)( v_i(1,\sminus)-v_i(0,\sminus)) + v_i(0,\sminus)$, which is a decomposable valuation with $\hat v_i(\profile) = \lambda(s_i)$, $h_i(\sminus) = v_i(1,\sminus)-v_i(0,\sminus)$ and $g_i = v_i(0,\sminus)$. This proves the forward direction of the lemma.
    
    For the converse direction, let $v_i(\profile) = \hat{v}_i(\profile)\cdot h_i(\sminus) + g_i(\sminus)$ and consider two signals $s,s'\in S_i$. For any $\lambda\in [0,1]$, we have
    $ 
     \lambda v_i(s,\sminus) + (1-\lambda)v_i(s,\sminus) = (\lambda \hat{v}_i(s,\sminus) + (1-\lambda)v_i(s',\sminus))\cdot h_i(\sminus) + g_i(\sminus).
    $
    
    Since $\hat{v}_i(\cdot,\sminus)$ is a continuous function from $S_i$ to $\reals$, by the intermediate value theorem there exists some $t\in S_i$ such that $\hat{v}_i(t,\sminus) = \lambda \hat{v}_i(s,\sminus) + (1-\lambda)\hat{v}_i(s',\sminus)$. Plugging this back into the decomposed formulation of $v_i$, we obtain 
    $
        v_i(t,\sminus) = \lambda \hat{v}_i(s,\sminus) + (1-\lambda)v_i(s',\sminus).
    $
    This proves that $D$ is a convex domain, concluding the proof of the lemma.
\end{proof}

%\vspace{1ex}
\noindent {\bf Connecting $f$-single-crossing and W-Mon. }
The following lemma now follows from %~\citet{ABMH10} and~\citet{CE02},
bullets (2) and (3) of Proposition~\ref{prop:IDV-implementability}, combined with Lemma~\ref{lem:convex-decomposable}.
 
\begin{lemma}\label{lem:wmon-implies-truthful-when-decomp}
Given any decomposable valuations $\vprofile$, a finite-valued social choice function $f$ is %ex-post \inbal{unify with other such statements} 
truthfully implementable if and only if $f$ satisfies weak monotonicity (W-Mon).
\end{lemma}

Recall that we {have already established} a stronger result in the previous section: in Theorem~\ref{thm:linear-characterization} we showed that for \emph{any} social choice function (potentially infinitely-valued), $f$-single-crossing is both necessary and sufficient for implementability under decomposable valuations. 

By Lemma~\ref{lem:wmon-implies-truthful-when-decomp} and Theorem~\ref{thm:linear-characterization}, 
we establish an equivalence between weak monotonicity and $f$-single-crossing under decomposable valuations for finite-valued $f$s.
The same holds for general $f$s by Lemmas~\ref{lem:sc-implies-weak-sc},~\ref{lem:weak-f-sc-to-wmon}, and \ref{lem:wmon-implies-f-sc-when-decomp}.

\begin{corollary}
\label{cor:SC-equiv-to-WMON}
For any IDV social choice setting with decomposable valuations $\vprofile$, it holds that a social choice function $f$ satisfies weak monotonicity (W-Mon) if and only if $\vprofile$ satisfies $f$-single-crossing  
\end{corollary}

\subsection{Decomposable Valuations form the Frontier of W-Mon Truthfulness}\label{sub:impossibility-for-non-decomposable}

An interesting implication that arises from the connection between decomposable valuations and convex domains is that decomposable valuations form the frontier of W-Mon truthfulness. The following theorem from \cite{ABMH10} shows that in IPV settings, when the domain is non-convex then W-Mon is insufficient for implementability.

\begin{theorem}[\citet{ABMH10}, Theorem 3]\label{thm:ashlagi-non-convex}
    Given any single-agent IPV social choice setting with a non-convex domain (which is not single-dimensional), there exists a finite-valued social choice function $f$ for which weak monotonicity (W-Mon) holds and yet $f$ is not implementable.
\end{theorem}

Lemma~\ref{lem:convex-decomposable} shows that for any valuation function $v$, the induced domain is convex if and only if $v$ is decomposable. Therefore, by applying Theorem~\ref{thm:ashlagi-non-convex} we obtain the following result. 

%They show that even for a single agent setting (which is trivially IPV), for each non-convex domain there exists a finite valued $f$ that satisfies weak monotonicity but is not truthfully implementable. We thus obtain the following result.

\begin{corollary}%[Decomposability is the frontier of W-Mon truthfulness]
\label{cor:impossibility-for-non-decomposable}
    For any non-decomposable valuation $v$ (which is not single-dimensional), there exists a social choice function $f$ for which weak monotonicity (W-Mon) holds and yet $f$ is not implementable.
\end{corollary}



This result implies that the class of decomposable valuations is the {\em frontier} of valuations in IDV settings for which weak monotonicity characterizes truthfulness. That is, for any valuation function that is non-decomposable, there exists a single agent example with some social choice function $f$, for which weak monotonicity is insufficient for implementability. Therefore, any class of valuations broader than decomposable valuations would require stronger conditions for implementability. 


==> arXiv version/intro.tex <==
\section{Introduction}

\noindent{\bf The interdependent values (IDV) model.} 
An underlying assumption in the vast majority of studies on mechanism design and social choice is that agents have independent private values \emph{(IPV)} for the different outcomes. 
And yet, in real-life scenarios, this is rarely the case. Indeed, in many auction settings, agent values are highly interdependent. A typical example is an auction for modern artwork, where an agent's value depends on others' assessment of the work's merit -- both since others may be better-informed on modern art, and since their opinions may determine the resale value of the work. 
Another canonical example is an auction for drilling rights, in which the information one
agent has about whether or not there is oil to be found is extremely relevant
to how another agent evaluates the rights being auctioned. 

The work of \citet{MW82} builds upon~\citet{Wilson77} to introduce the {\em interdependent value} model \emph{(IDV)}, which captures such interdependencies of values among the agents. 
This work was recently recognized by the Nobel prize in economics, awarded in 2020 to Milgrom and Wilson~\citep{Nobel20}. 
In the IDV model, every agent~$i$ has a privately-known signal $s_i$ that captures the agent's information about the different outcomes, in addition to a publicly-known valuation function that maps the signals of \emph{all} $n$ agents to $i$'s values for the outcomes.
The importance of this model is in providing a much more accurate depiction of valuations in practice -- for example, it sheds light on well-known phenomena like the winner's curse, which cannot be explained under IPV~\cite[e.g.,][]{ChenEW22}. 

\vspace{1ex}
\noindent{\bf IDV and welfare maximization.} 
The IDV model also raises fascinating theoretical challenges:
An important theme of algorithmic game theory is the interplay between truthful implementability and the approximation factor achievable for a certain optimization problem. In IPV this has been extensively studied for the objective of minimizing makespan, with a recent breakthrough showing a large gap between non-truthful and truthful approximation (even with no computational limitations)~\citep{ChristodoulouKK21}. For arguably the most natural objective -- welfare maximization -- there is no gap in IPV due to the VCG mechanism (computational considerations aside), which applies beyond auction settings to general social choice. In IDV however, such a gap exists even for welfare in auction settings.

The economics literature has studied conditions under which welfare maximizing auction design is possible in the IDV model. 
For single-dimensional settings, if valuations satisfy a condition called {\em single-crossing}, one can obtain the maximum welfare in an (ex-post) truthful mechanism \citep{Ausubel99}.
Recently, work in computer science has combined approximation with alternative assumptions to extend positive welfare results beyond single-crossing. \citet{EFFGK19} achieve a constant-factor approximation for valuations satisfying {\em submodularity over signals (SOS)}. They extend their result under \emph{separability} even to multi-dimensional settings. 

\vspace{1ex}
\noindent{\bf Public projects with IDV.} 
Beyond auction design, for more general social choice settings, the state of affairs is less clear. A well-studied such setting is the \emph{combinatorial public projects problem (CPPP)}, in which a set of resources is chosen to \emph{collectively} serve a community~\citep{BuchfuhrerSS10,SchapiraS08,LucierSST13,Markakis17,Dughmi11,DughmiRY16}. 
This captures various real-world resources ranging from roads to communication networks. In fact, CPPP can be shown to essentially capture any social choice setting (computational considerations aside -- see Section~\ref{sec:approximation}).
The motivation to study such settings is more relevant than ever given the current trend towards allowing communities more influence over public policies and public decision-making~\cite[e.g.,][]{BrandlBP+21}.
The purpose of this paper is to initiate the study of mechanism design for public projects under IDV. 

We briefly describe the CPPP setting and provide a running example (Example~\ref{eg:running}): There are $n=2$ agents and a pool of $m=3$ potential public projects, including building a new bridge, opening a library, and building a train station. The goal is, for a given $k\le m$, to choose which $k$ projects to realize in order to maximize social welfare. Every agent $i$ has a privately-known signal $s_i\in\reals^+$ capturing their private information about the projects. The value $v_{ij}$ of agent $i$ for project $j$ is an increasing function of all signals $s_1,\dots,s_n$. In Example~\ref{eg:running}, the values are simple linear functions, but more generally they can be \linear, polynomial, etc. 
Observe that despite the fact that the signals are single-dimensional, the value space of every agent is multi-dimensional (and the related complexities apply).

\begin{example}[Running example]
\label{eg:running}
We define a public projects instance with 
$n=2$ agents and $m=3$ potential projects, with the following values:
\begin{itemize}
    \item Agent 1's values: $v_{11} = 3s_2$, $v_{12} = \frac{s_1}{2}+ s_2$, $v_{13}=2s_1$.
    \item Agent 2's values: $v_{21} = s_2$, $v_{22} = s_1+ \frac{s_2}{2}$, $v_{23}=0$.
\end{itemize}
(Figure \ref{fig:three-linear-projects-with-single-crossing} in Section~\ref{sec:linear-characterization} depicts the values of agent 1 for the three projects as a function of her signal $s_1$, when agent 2's signal is fixed to $s_2=1$.)
\end{example}

\noindent{\bf Overview of our contribution.} Inspired by the study of welfare maximization for auctions with IDV, for public projects we explore the two known conditions under which positive results are attainable for auctions: single-crossing valuations, and SOS valuations. In both cases, the existing theory falls short of solving the public projects setting. 
Our contribution is twofold: (i)~We give useful characterizations of truthful mechanisms for public projects in IDV settings (Section~\ref{sec:linear-characterization}, complemented by Section~\ref{sec:general-charac}); (ii)~We provide possibility and impossibility results for welfare approximation in such settings (Section~\ref{sec:approximation} -- this stand-alone section can be referred to directly by the interested reader).
Beyond the concrete results, our study reveals interesting connections between properties (e.g.~single-crossing and W-Mon) that were previously studied separately in the truthful implementability literature. %We now turn to a more detailed account of our contributions.
%\inbal{add organization, say sec 4 is standalone}

%\inbal{Do we want to add a natural PP example where $f$-single-crossing holds for welfare?}

\subsection{Characterization of Implementability in IDV}
%\inbal{From the meeting: simplify the message of Section 3. Focus on decomposable valuations, state the thm, state we have additional results beyond these valuations - details are deferred to Sec 3, in the figure there is a full picture. What are these valuations, what we show for them, prev lit.}
In much of the previous IDV literature the focus has been on single-dimensional settings and welfare maximization. It is well-known that in this case, the valuations need to satisfy a condition called single-crossing to obtain optimal welfare truthfully~\citep[e.g.][]{Maskin92,Ausubel99,DM2000,JehieM01}.
%\michal{missing references}\divya{are these good?}. 
We go beyond both single-dimensional settings and the social welfare objective.

\vspace{1ex}
\noindent{\bf Single-crossing-based characterization for decomposable valuations. }
In Section~\ref{sec:linear-characterization} we develop a useful characterization as follows. We first study \emph{\linear} valuations -- for each agent $i$, valuation $v_i$ is linear as a function of $s_i$. We define a necessary and sufficient condition for truthful welfare maximization beyond single-dimensional settings, termed \emph{strong} single-crossing. This condition is based on a comparison of slopes between an agent's valuation and the social welfare of different outcomes. 
%the slopes of the valuation of an agent, and the social welfare of different outcomes. 
We can extend \linear to a general valuation class we refer to as \emph{decomposable}. A valuation is decomposable if the influence of agent $i$'s signal $s_i$ on her value $v_i$ is independent of the social choice outcome. This class of valuations encompasses many standard examples of interdependence studied in the literature, such as the resale model~\citep{MW82} or the wallet game~\citep{Klemperer1998}, and generalizes {previously studied classes of valuations such as fully linear valuations (for which~\citet{JehieM01} provide a characterization)} and separable valuations~\citep{MookherjeeR92} (for which \citet{CE02} give a characterization). 
% Moreover, the fact that the valuations are \linear is only useful to us in that, for each agent $i$ and signal profile $\sminus$, the ordering of the slopes of $v_i$ of different outcomes with respect to $s_i$ is the same for all possible signals $s_i$. %This too can be generalized to a much broader class of valuations in which the slopes of the values for different outcomes always have {a global} ordering. %between outcomes. 
% We identify a broader class of valuations that satisfies this condition and term it \emph{decomposable}.
% %\avi{Notice that all SOS separable valuations are also decomposable (but not the other way around). Therefore, the class for which \citet{EFFGK19} provide a 4 approximation is a subclass of our decomposable valuations class. This solidifies the fact that this class of valuations is interesting and important.}\avi{This comment is actually WRONG: SOS separable valuations and decomposable valuations are incomparable classes}
% In a decomposable valuation, the influence of agent $i$'s signal $s_i$ on her value $v_i$ is independent of the outcome. %The intuition is that in many cases an agent's signal affects her value in a similar way across outcomes; for example if the signal encodes her personal expertise then this information is likely to be taken into account in a correlated way.
% This class encompasses many standard examples of interdependence in the literature such as the resale model~\citep{MW82} and the wallet game~\citep{Klemperer1998}.
% Besides multi-linear, this class also generalizes the class of separable environments~\citep{MookherjeeR92} (for which \citet{CE02} have a similar characterization). 
%\michal{I changed cite to citep in the last two citations. We have to make a pass to check if there're other places that need a fix. I'll change the ones that I see as I make my pass, but one needs to make a global search}
%Additionally, we can go beyond the comparison of deterministic outcomes to an analogous comparison between any two distributions on the set of outcomes. This allows us to characterize the implementability of any randomized social choice function.
Finally, to go beyond welfare maximization to any social choice function $f$ over decomposable valuations, we generalize strong single-crossing to $f$-single-crossing. To summarize:

\vspace{0.1in}
\noindent {\bf Theorem:} (See Theorem \ref{thm:linear-characterization})
For any decomposable valuation profile $\vprofile$, a social choice function $f$ is (ex-post IC-IR) implementable if and only if $\vprofile$ satisfies $f$-single-crossing.

\vspace{0.1in}
\noindent\textbf{Beyond decomposable valuations.} In Section~\ref{sec:general-charac} we first complement our useful characterization from Section~\ref{sec:linear-characterization} by providing a characterization beyond decomposable valuations.
{Namely, we show that \emph{weak} $f$-single-crossing is a necessary and sufficient condition for implementability in IDV settings. Like other general characterizations (e.g.~for general IPV social choice), this condition is not easy to utilize.} 

{We then study the connections between IPV and IDV implementability through the framework of~\citet{CE02}. Combining these with the results of Section~\ref{sec:linear-characterization} paints a comprehensive picture of the complex landscape of implementability.} 
The connections between the multitude of characterizations are summarized in Figure~\ref{fig:high-level-scheme}. Notably, our results establish that in the setting of decomposable valuations, \emph{all} the conditions depicted in Figure~\ref{fig:high-level-scheme} are equivalent. This provides an arguably surprising formal connection between single-crossing conditions for IDV, and W-Mon/C-Mon characterizations for IPV, which were previously studied separately in the literature. It also shows the importance of the class we have defined of decomposable valuations --- we prove the equivalence does not hold beyond it. In other words, decomposable valuations are the frontier for which a workable characterization of implementability exists, similar to convex domains for IPV which form the frontier between W-Mon (workable) and C-Mon characterizations.
%\michal{The above paragraph replaces the following commented out text.}
%to characterize implementability in IDV settings. We call this condition \emph{weak $f$-single-crossing}. However, while general, this condition is much harder to work with than $f$-single-crossing. 

% $f$-single-crossing implies weak $f$-single-crossing, therefore it is a sufficient condition in IDV settings in general. %However, we observe that, any class of valuations beyond decomposable valuations contains an example of a social choice function for which $f$-single-crossing does not hold, yet weak $f$-single crossing holds showing that it is not a necessary condition beyond decomposable valuations. %
%An illustration of the connections between different notions of single-crossing is provided in Figure~\ref{fig:high-level-scheme}. %\avi{This is not the result implied by Ashlagi et al. We do not have this result (though I think it is perhaps obvious...). What Ashlagi et al. tells us is that *WMON* is not sufficient beyond decomposable valuations. This is a bit confusing because WMON is a necessary and insufficient condition, while $f$-single-crossing and a sufficient yet not necessary condition...}

% \vspace{1ex}
% \noindent{\bf Connections to IPV implementability. }
% Interestingly, we find that our conditions are related to monotonicity notions studied in IPV, namely, weak monotonicity (W-Mon) and cycle monotonicity (C-Mon). A different way to obtain a characterization in IDV settings is by the Chung-Ely  equivalence of IDV and IPV \citep{CE02}. Essentially, Chung-Ely's equivalence says that any necessary (resp. sufficient) condition in the IPV setting can be naturally translated into a necessary (resp. sufficient) condition in the IDV setting.

% In particular, by \citep{ABMH10}, in \emph{convex domains} in the IPV setting, weak monotonicity is sufficient for implementability for finite-valued $f$. Furthermore, \citet{ABMH10} show that for any single agent setting with a non-convex domain, there exists a social choice function $f$ that satisfies weak monotonicity but is not implementable.

% We show that, in the IDV translation, convex domains are induced by (and only by) decomposable valuations (see Lemma \ref{lem:convex-decomposable}). Thus, the \citet{CE02} equivalence establishes that, for decomposable valuations, weak monotonocity is sufficient for finite-valued $f$; and we see that, for decomposable valuations, $f$-single-crossing is equivalent to weak monotonicty. Thus, our results for decomposable valuations through $f$-single-crossing are in fact stronger than those obtained through \citet{ABMH10}, because we show that weak monotonicty is sufficient for \emph{any} social choice function. Moreover, applying the negative result from \cite{ABMH10} we conclude that our results are also tight in some sense. As for any class of valuations broader than decomposable valuations, there exists a single agent example where a monotone social choice function is not implementable.

% \vspace{0.1in}
% \noindent {\bf Theorem:} (See Theorem~\ref{thm:impossibility-for-non-decomposable})
% %\avi{The first part of this theorem follows immediately from the fact that weak monotonicity implies $f$-single-crossing for decomposable valuations. It is completely unrelated to the discussion in this part of the section. I think we should make the theorem just about the impossibility result: showing that decomposable valuations are ``tight'' in some sense}
% %For any decomposable valuation profile, the social choice function $f$ is ex-post IC and ex-post IR implementable if and only if weak monotonicity holds. Moreover, 
% %
% For any non-decomposable valuation, there exists a single agent social choice function $f$ such that $f$ is weakly monotone and yet $f$ is not implementable.
% \vspace{0.1in}



%------------------- FIGURE: CHARACTERIZATIONS DIAGRAM ----------------------%
\begin{figure}
    \centering
    %\resizebox{1\textwidth}{!}{%
        \input{EC 2022/figures/high-level-diagram.tex}
     %   }
    % Pre-compiled image file: (Uncomment to make compilation time faster)
    %\includegraphics[]{EC 2022/figures/high-level-diagram.pdf}
    \caption{A scheme of the connections between implementability characterizations.\\
    For example, the scheme shows the equivalence between $f$-single-crossing and W-Mon for decomposable valuations (see the ``triangle'' of arrows formed on the bottom-left). It further shows that the $f$-single-crossing property characterizes implementability for decomposable valuations in the IDV model (see the middle ``line'' of arrows from left to right). See Sections~\ref{sec:linear-characterization} and \ref{sec:general-charac} for details. %W-Mon is arguably the best-known characterization from the classic IPV literature. 
    \\{\textsuperscript{\textdagger}Single-crossing is defined for single-dimensional settings. \\\textsuperscript{*}Strong single-crossing and $f$-single-crossing are defined for decomposable valuations (see Observation~\ref{obv:decomposable-ssc-fsc}).} 
    }
    \label{fig:high-level-scheme}
\end{figure}
%----------------------------------------------------------------------------%

%\michal{strong single-crossing is not mentioned above, and yet, we're using it in our first sentence in the next subsection.}

%\noindent{\bf Approximate Welfare for Public Projects}
\subsection{Approximate Welfare for Public Projects}
%\divya{Cite SODA'21 private valuations IDV, literature by David Parkes' group, Dasgupta-Maskin.}
By our characterization results in Section~\ref{sec:linear-characterization}, for any public project instance with decomposable valuations, if strong single-crossing is satisfied then the optimal welfare can be obtained by a truthful mechanism. 
In Section~\ref{sec:approximation} we study settings without strong single-crossing.

Our first observation is that welfare maximization in auctions with $k$ identical items can be reduced to welfare maximization in public projects (choosing $k$ projects).
With this reduction in hand, known impossibility results in auction design (see \cite{EFFG18,EFFGK19}) immediately imply the following inapproximability results in public projects, even in cases where a single project should be chosen. 
First, no welfare approximation guarantee can be provided by any deterministic truthful mechanism.
Second, in the absence of additional constraints, no randomized mechanism can give any non-trivial (i.e., better than $1/m$) welfare approximation. 

\citet{EFFGK19} recently proposed to circumvent these impossibilities in auction design by considering valuations that satisfy a natural property called {\em submodularity over signals} (SOS).
Roughly speaking, these are valuations where the increase in one's value due to an increase in her signal is smaller when other signals are higher.
SOS is a natural condition that holds in essentially all examples in the IDV literature.
\citet{EFFGK19} showed that if valuations are  separable\footnote{{A valuation function $v_i : \mathcal{A}\times \mathcal{S} \to \reals^+$ is separable if there exist functions $h_i: \mathcal{A}\times S_i \to \reals^+ $ and $g_i: \mathcal{A}\times \mathcal{S}_{-i} \to \reals^+$ such that $v_i(a;\profile) = h_i(a;s_i) + g_i(a;\sminus)$}.} SOS, then one can obtain $4$-approximation even in general combinatorial auctions.

Does SOS come to our rescue in public projects as well?
{Unfortunately, SOS does not suffice for providing welfare guarantees in public project settings.}
Our main impossibility result is that even under separable SOS (linear) valuations, no  universally truthful mechanism can perform better than allocating a project at random. 

\vspace{0.1in}
\noindent {\bf Theorem:} (see Theorem~\ref{thm:lower-bound})
There exists a public projects instance with separable SOS valuations for which no universally truthful mechanism can give better than $1/m$ approximation to %the social
welfare.
\vspace{0.1in}

What is the source of the difference between auctions and public projects? 
A key component in the mechanism for auctions is a random partitioning of the agents into two groups of agents: those who are included and those who are excluded. 
The challenge in public projects is that once a project is in place, agents cannot be excluded from using it. 
However, an interesting subtype of public projects is the class of excludable public projects, often termed {\em club goods} in the economics literature \citep{Buchanan1965}. 
Examples of club goods include libraries, cinemas, swimming pools, or any public facility that benefits a restricted group of members. 

Our main positive result is that the truthful mechanism tailored for auctions in the IDV setting {\citep{EFFGK19}} can be adapted to excludable public projects.
This result greatly extends the mechanism's applicability.

\vspace{0.1in}
\noindent {\bf Theorem:} (see Theorem~\ref{thm:4-approx})
There is a universally truthful mechanism that gives $1/4$-approximation to welfare for excludable public projects with separable SOS valuations.
\vspace{0.1in}

A conceptual takeaway from our results is that exclusion is an important tool for welfare approximation guarantee in IDV settings.
In particular, our strong impossibility results may suggest that the strong notion of exclusion used in auction settings, where some agents are totally excluded, is inevitable.
%While exclusion may be perceived as more natural for auction settings, the mechanism in \cite{EFFGK19} uses a stronger notion exclusion, where some agents are totally excluded. 
%Our strong impossibility result may suggest that this is inevitable.

\vspace{1ex}
\noindent{\bf Open problems.}
%\inbal{From meeting: Organize this better; maybe generalize some questions / be more concrete, different order, so it's not like brainstorming}
Our work suggests many natural directions for future research. 
\emph{First}, providing improved approximations or giving tighter bounds: Can we improve our $\frac{1}{4}$ approximation algorithm, perhaps by allowing randomized mechanisms that are truthful in expectation rather than universally truthful? Does the impossibility result of Theorem~\ref{thm:lower-bound} that necessitates excludability hold for truthful in expectation mechanisms? Can we show that the exclusion step at the beginning of the SOS mechanism is necessary not just for public projects but even for auctions?
%How do we even formally capture the notion of impossibility ``without exclusion'' in auctions?
\emph{Second}, relaxing assumptions: For example, is the separable SOS assumption necessary for a constant-factor approximation for public projects? (The same question is still open for auction design as well.)  
\emph{Third}, extending our results to related models: E.g., what is a characterization for truthfulness in IDV \emph{Bayesian} settings (i.e., with priors over the signals)? Can we design truthful mechanisms for other/additional objectives such as revenue maximization or budget balance? \emph{Fourth}, computational results: While our main focus is implementability rather than computation, we do get a polynomial-time truthful approximation algorithm for CPPP with IDV under additive valuations. A truthful solution to CPPP is APX-hard even for IPV for more general valuations~\citep{PSS08}. What approximation factor is tractable for CPPP with IDV beyond additive valuations?
%
%Can we expand the impossibility result to show that the random mechanism in the SOS paper is the right and the only thing to do, in order to get lower bounds? 
%lower bound of computation 
%if values are not additive for different projects -- submodular etc.
%\michal{Where does the above paragraph belong?}

%Stuff to add: ``SOS does not rescue us''. There was no single crossing for multi-dim before. highlight more that SC is monotonicity.

%In fact, putting aside computational considerations, PP is as general as the most general form of social choice (an outcome can be seen as a project).

%The public project setting is the most general single-parameter social choice setting (?).

\subsection{Additional Related Work}

\vspace{1ex}
\noindent{\bf Interdependence.}
\citet{CE02} show a connection between IPV and IDV truthfulness characterizations -- for completeness we include this as Lemma~\ref{lem:Chung-Ely} below. This enables importing to IDV characterizations for IPV, including the works of \cite{LMN03,BikhchandaniCS03,GuiMV04,SaksY05} on weak monotonicity (W-Mon). 
%\citet{JehieM01} study welfare maximization under \emph{Bayesian} truthfulness -- we leave Bayesian settings for future research.

%\inbal{From meeting: give 2 sentences on the main result of each paper. Mention the other model -- }
%%%\avi{Lavi et al. have a very restricted characterization. Only for order based domains. With known valuations order based domains contain only trivial examples (e.g. when the value of all outcomes is the same) and thus the Lavi et al. characterization is not applicable to our model, even when using Chung-Ely equivalence }
%\todo{We currently have no mention of CMON and convex domains...}
%The classic model of interdependent values was introduced by Milgrom and Weber \cite{MW82}. 
The bulk of algorithmic work on mechanism design has focused
on the IPV model. Early ventures beyond this model considered private values that are \emph{correlated} \citep[e.g.,][]{DobzinskiFK15}.
\citet{RT16} suggested to apply the computer science lens to the study of
mechanisms for interdependent values. They unified and generalized previous results to establish technical foundations for this study, including a characterization of truthful mechanisms for single-parameter settings with IDV. They also demonstrated natural sufficient conditions under which positive results in the form of robust mechanisms for approximate revenue maximization can be achieved. Concurrently, \citet{Li17} developed a simple near-optimal auction for revenue maximization with IDV, namely, the VCG mechanism with monopoly reserves, assuming monotone hazard rate value distributions.
% in the context of revenue maximization \michal{Why is it important that it is in the context of revenue maximization? characterization is separate from the objective function};
\citet{ChawlaFK14} studied revenue approximation under relaxed assumptions.
They introduced a variant of the generalized VCG auction with reserve prices and random admission, and showed that this auction gives a constant approximation to the optimal expected revenue under a submodularity assumption on the valuation functions.

{There has also been work on multi-dimensional settings and multi-dimensional signals. \citet{JehieM01} study a general social choice setting with multi-dimensional signals %space \avi{remove the word ``space''?} (where each agent $i$ has a multi-dimensional signal $s_i$)
under fully linear valuations where $v_{i}(a;\profile) = \sum_{j=1}^n \alpha_{ij}^a\cdot s_{ij}^a$ for each agent $i$. 
They consider a multi-dimensional signal space, compared to our single-dimensional signal space. 
On the other hand, they consider fully linear valuations, which is a special case of decomposable valuations considered in our work. They provide a characterization for Bayesian incentive compatibility, which translates to our $f$-single-crossing definition in the single-parameter signal regime (when applied to fully linear valuations). \citet{JehielMMZ06} showed that the constant social choice functions are the only deterministic social choice functions that are implementable in general multi-dimensional IDV settings with multi-dimensional signals and transferable utilities.}
%Chung and Ely 
% ex-post incentive compatible public decision rules. Their characterization extends characterizations under independent settings to interdependent settings. This allows us to combine \cite{CE02} and \cite{LMN03} to obtain our characterization. Moreover, \cite{CE02} do not consider SOS and excludability which we study in this paper.

The above studies and much of the other work on interdependent values assumed a single-crossing condition \citep[e.g.][]{MW82, dG82, Ausubel99, DM2000, BSV09, CKK15} (see also~\cite{WikiSingleCrossing22}).
%%%\avi{I copied this list of papers from somewhere else... Need to make sure it actually makes sense.}
Interdependent values with relaxed single-crossing were first studied by \citet{EFFG18} with a focus on welfare.
Interdependence without any single-crossing condition was studied by \citet{EFFGK19}, who introduced the submodularity over signals (SOS) condition. There is also a literature relaxing the knowledge assumption on the valuation functions themselves (in addition to the signals, which are privately-known by design in the IDV model). In \citep{DM2000,RobuPIJ13} the valuations are unknown only to the \emph{designer}; in \citep{EGZ22} they are unknown to the other agents as well (each agent knows only her own valuation). 

The described works on interdependence are in the context of auctions; we now turn to public projects which were studied for the IPV model.
%The first work that studies interdependent values without single-crossing is \cite{EFFG18}. 

%A followup work by a superset of the authors, \cite{EFFGK19}, introduced the notions of SOS and the random exclusion mechanism we make use of in this paper. Our paper studies the setting of interdependent public projects (rather than auctions) both under the assumption of a Single-Crossing condition (which we introduce and adapt to the public projects setting), and without the assumption of such a condition. 

\vspace{1ex}
\noindent{\bf Public projects.}
%\inbal{@Divya and @Michal, please check my new organization of the paragraph and new reference:}
%Papadimitriou, Schapira and Singer 
Public projects have long been studied in economics, with main objectives of welfare maximization and budget balancedness~\cite{Moulin94}.
%Cost sharing (dobinski et al.) --- this connects well to "excludable"/"club goods".
%Econ literature on club goods.
%In AGT the computational hardness of such settings was studied\divya{maybe remove this sentence?}. 
\citet{PSS08} study the hardness of the Combinatorial Public Projects Problem (with independent, multi-parameter valuations), measured by both communication complexity and computational complexity.
A related but different body of AGT literature returns to the problem of cost sharing \citep{DMRS08, DO17} via approximation. In these settings each public project has a cost and the goal of the mechanism is to maximize welfare under the constraint that it must cover the costs of the chosen projects using the payments of the agents. %Typically the setting is that there is one public good with some fixed cost, and the goal is to maximize welfare while ensuring the payments of the agents cover the cost of the public good (otherwise, the mechanism designer may choose not to provide the public good at all)\divya{I am confused by this, isn't there an impossiblity result that we can't get both welfare max and BB?}. 
The property of excludability is inherent to the model, since cost sharing implies that agents on which the mechanism does not impose a cost for a given project should not be able to enjoy the benefits of that project. 
%
The topic of excludable public goods was studied extensively in the economics literature \citep{DR99a, DR99b}, sometimes referred to as club goods \citep{Buchanan1965}. 
%%%\avi{add more econ papers}. 
 Our paper extends this well-studied setting to multiple public goods and interdependent values (while we do not consider the cost of projects nor the aspect of budget-balancedness).

==> arXiv version/multi-linear.tex <==
\section{Implementability Characterization for Decomposable
Valuations} %(and an Extension to Decomposable)}
\label{sec:linear-characterization}
% \inbal{the previous version sounded like an extra condition}
In this section we first study necessary and sufficient conditions for truthful implementation of a social choice function for IDV settings with \linear valuations. {In Section~\ref{sec:warm-up-welfare} we define a strong single-crossing property that is necessary and sufficient for truthful welfare maximization, and in Section~\ref{sub:linear-characterization} we generalize this to a necessary and sufficient condition for implementability of any social choice function $f$. {We observe that the ``decomposability'' property of \linear valuations is what drives this characterization.} Indeed, in Section~\ref{sec:decomposable} we show that the characterization of Section~\ref{sub:linear-characterization} extends to the more general class of {\em decomposable} valuations.}
%\inbal{from meeting: ``slopes'' not clear; add other subsections}
%\michal{what's the status of this comment of inbal?}

\subsection{Warm-Up and Illustrations: Welfare Maximization for Auto-linear Valuations}\label{sec:warm-up-welfare}
In this section {we study truthful welfare maximization} and provide intuition for our generalization of single-crossing towards a characterization of truthfulness.
%As a first step, we study a con
%\linear valuations. %Namely, valuations where for each agent $i$, the valuation $v_i$ is linear as a function of $s_i$.
%In this setting, the characterization condition, which we call \emph{strong single-crossing}, holds whenever the slopes of the social welfare of each outcome are consistent in ordering with the slopes of every agent's valuation of each outcome.
%
We define a condition similar to single-crossing that is necessary and sufficient for truthful welfare maximization beyond single-dimensional settings. Our single-crossing condition, {termed} \emph{strong single-crossing}, is based on the comparison of the slopes of an agent's valuation and the slopes of the social welfare for different outcomes. For instance, in Example~\ref{eg:running}, the slopes of agent $1$'s valuations with respect to $s_1$ are $0,\frac{1}{2}$, and $2$ for the projects $1,2$, and $3$ respectively, and the slopes of the social welfare with respect to $s_1$ are $0,\frac{3}{2}$, and $2$ for the projects $1,2$, and $3$ respectively. Notice that, when considering the projects in increasing order with respect to either the slopes of the valuation or the slopes of the welfare we obtain the same ordering, i.e., $1<2<3$. This consistency in the order of slopes is the essence of our single-crossing condition (when it holds for each agent $i$ with respect to signal $s_i$).


{Other studies have considered similar strong single-crossing conditions for truthful welfare maximization, for example,~\citet{DM2000} define a stronger condition for general multi-item auctions,{~\citet{JehieM01} define this for general social setting under fully linear valuations},~\citet{CE02} define this for \emph{separable environments} (which is non-comparable to multi-item auctions), and~\citet{ItoP06} apply it to auctions with single-minded bidders (which is a separable environment).}


%\michal{I debate whether it would be good to add a definition of strong SC already in this subsection. We keep referring to this condition without ever providing a definition. The definition appears only in section 3.2.}

\begin{definition}[Strong single-crossing]\label{defn:linear-single-crossing}
 Given any IDV social choice setting $(n,\mathcal{S}, \mathcal{A},\vprofile)$ with \linear valuations $\vprofile$. Let $\Wel(a;\profile) = \sum_{i} v_i(a; \profile)$ denote the welfare of allocation $a\in \mathcal{A}$ given signal profile $\profile$.
 We say that $\vprofile$ satisfies strong single-crossing, if for each $i\in [n]$ and $\sminus\in \mathcal{S}_{-i}$
 \[
     \pdif{\Wel}{s_i}(a_1;\profile)\le \pdif{\Wel}{s_i}(a_2;\profile) \le \ldots \le \pdif{\Wel}{s_i}(a_r;\profile)
 \]
 implies
 \[
    \pdif{v_i}{s_i}(a_1;\profile)\le \pdif{v_i}{s_i}(a_2;\profile) \le \ldots \le \pdif{v_i}{s_i}(a_r;\profile),
 \]
 where $a_1,\ldots, a_r$ denote all the outcomes such that $a_j \in \max_{a\in \mathcal{A}} \Wel(a;z,\sminus)$ for some $z \in S_i$.
\end{definition}

\begin{observation}\label{obv:single-sc and strong-sc}
Applying the strong single-crossing condition to single-item auctions would mean that $\pdif{\Wel}{s_i}(i,\profile) \ge \pdif{\Wel}{s_i}(j,\profile)$ for all $i,j$, because $\pdif{v_i}{s_i}(i;\profile) \ge 0 = \pdif{v_i}{s_i}(j;\profile)$. Since by definition $\Wel(i;\profile) = v_i (i,\profile)$, that is exactly the same as the single-crossing condition $\pdif{v_i}{s_i}(i,\profile) \ge \pdif{v_j}{s_i}(j,\profile)$ from Definition~\ref{def:sc-auctions}.
\end{observation}

%\michal{Is $W$ in the observation above supposed to be $Wel$?}
{Observe that for any \linear valuations $\vprofile$, for all outcomes $a$ and signal profile $\sminus$, the slopes with respect to $s_i$, $\pdif{v_i}{s_i}(a;\profile)$ and $\pdif{\Wel}{s_i}(a;\profile)$, is a constant with respect to $s_i$. 
%In other words, for any agent $i$ and signal profile $\sminus$, the slopes of $v_i$ and $\Wel$ with respect to $s_i$ induce the same ordering over outcomes for all signals $s_i \in S_i$.
}


\vspace{1ex}
\noindent{\bf A visual illustration of strong single-crossing.}
The reason this condition implies implementability can be illustrated visually. 
Recall Example~\ref{eg:running}, where there are
$n=2$ agents and $m=3$ potential projects with the following values:
\begin{itemize}
    \item Agent 1's values: $v_{11} = 3s_2$, $v_{12} = \frac{s_1}{2}+ s_2$, $v_{13}=2s_1$.
    \item Agent 2's values: $v_{21} = s_2$, $v_{22} = s_1+ \frac{s_2}{2}$, $v_{23}=0$.
\end{itemize}
The plot in Figure \ref{fig:three-linear-projects-with-single-crossing} (left) depicts this for $i=1$ and $s_2=1$ ($j_\ell=\ell$ for $\ell\in[3]$), where $f$ is welfare maximization. The blue region ($s_1\in[0,5/3]$) is when project $1$ maximizes welfare; the red region ($s_1\in[5/3,3]$) is when project $2$ maximizes welfare; and the green region ($s_1 \geq 3$) is when project $3$ maximizes welfare.
Notice that if we order the projects by the slope of the welfare with respect to $s_1$ we get back the order of the projects that maximize welfare as $s_1$ increases. Moreover, the same order of slopes would be obtained when considering the valuation of agent $1$ for each of the projects. 
The fact that the slopes are aligned allows us to define prices such that the utility maximizing project is also the welfare maximizing project for each signal $s_1$. This is illustrated in the plot on the right, where the arrows depict the shift in the values induced by the prices.

\vspace{1ex}
\noindent{\bf Strong single-crossing is necessary.}
Conversely, without having the slopes of $v_i$ with respect to $s_i$ ordered ``consistently'', i.e., when single-crossing does not hold, this is not possible. No set of prices can shift the lines such that the welfare maximizing outcome would also be the utility maximizer of agent $i$ for every signal $s_i$. This is illustrated in Figure \ref{fig:two-linear-projects-without-single-crossing}. The plot on the left depicts the utility of two projects as a function of $s_i$ (having fixed some set of signals $s_{-i}$ for the remaining agents). The blue and red lines depict $v_i$ for projects $j_1$ and $j_2$, respectively. The blue and red regions are the regions where project $j_1$ and $j_2$ maximizes welfare, respectively. Notice that the red line has a steeper slope than the blue line whereas the red region is to the left of the blue region --- the ordering is inconsistent! It is now easy to see that due to this discrepancy in the ordering, no set of prices can simultaneously place the blue line above the red line in the blue region and the red line above the blue line in the red region. Any price that shifts the red line below the blue line in the blue region would necessarily do the same in both regions. Similarly, a set of prices that ensure the red line is at the top in the red region would necessarily put it at the top in both regions. 

%------------------------ FIGURE: TRUTHFUL LINEAR ---------------------------%
\begin{figure}
\begin{center}
    \resizebox{\textwidth}{!}{%
    %\includegraphics{EC 2022/figures/three-projects.pdf}
    \input{EC 2022/figures/three-projects.tex}
    }
    % \includegraphics[height=5.5cm]{EC 2022/figures/three-projects-no-prices.png}
    % \quad
    % \includegraphics[height=5.5cm]{EC 2022/figures/three-projects-with-prices.png}
\end{center}
    \caption{Truthful prices in an \linear setting with three projects where $f$-single-crossing holds.} %Projects $j_1, j_2$ and $j_3$ are depicted in colors blue, red and green, respectively. The background color indicates the project chosen by the social choice function $f$. On the left plot, the colored lines indicate the value of agent $i$ for each of the projects. On the right plot, the colored lines indicate the utility for agent $i$ for each of the projects given their prices, and the faded lines indicate the original values from the plot on the left. Notice that the prices re-position the colored lines such that the topmost line at every point is in the color chosen by the social choice function $f$.}
    \label{fig:three-linear-projects-with-single-crossing}
\end{figure}
%-----------------------------------------------------------------------------%

%----------------------- FIGURE: LINEAR NO SC --------------------------------%
\begin{figure}
\begin{center}
    \resizebox{\textwidth}{!}{%
    %\includegraphics{EC 2022/figures/two-projects.pdf}
    \input{EC 2022/figures/two-projects.tex}
    }%
    
    % \includegraphics[height=3.5cm]{EC 2022/figures/two-projects-no-prices.png}
    % \includegraphics[height=3.5cm]{EC 2022/figures/two-projects-bad-red-price.png}
    % \includegraphics[height=3.5cm]{EC 2022/figures/two-projects-bad-blue-price.png}
\end{center}
    \caption{An \linear setting with two projects where $f$-single-crossing does not hold.} %Project $j_1$ and $j_2$ are depicted in colors blue and red, respectively. The background color indicates the project chosen by the social choice function $f$. On the left plot, the colored lines indicate the value of agent $i$ for each of the projects. On the center plot the changed red line indicates the utility of agent $i$ for project $j_2$. Notice that any price that makes the red line go below the blue line in the blue region would also make the red line go below the blue line in the red region. On the right plot, the changed blue line indicates the utility of agent $i$ for project $j_1$. Notice that any price that makes the blue line go below the red line in the red region would also make the blue line go below the red line in the blue region.}
    \label{fig:two-linear-projects-without-single-crossing}
\end{figure}
%------------------------------------------------------------------------------%

{Hence we get the following proposition characterizing efficient mechanisms for IDV settings with \linear valuations. We defer the proof to the appendix, where we provide a characterization for objective functions beyond welfare maximization.}

\begin{proposition}\label{prop:linear-characterization}
   For any IDV social choice setting $(n,\mathcal{S},\mathcal{A},\vprofile)$ with \linear valuations $\vprofile$, there is an ex post IC-IR mechanism that achieves optimal social welfare if and only if $\vprofile$ satisfies the strong single-crossing condition and the following payment identity holds for every $i$ and $\sminus$:
\begin{align*}
     p_{i}(x_j, \sminus) &= p_{i}(x_{j-1}, \sminus) + v_{i}(a_j; x_j) - v_{i}(a_{j-1};x_j) \\
     p_{i}(s_i, \sminus) &= p_{i}(x_j, \sminus) \quad \text{ for all } s_i \in [x_{j}, x_{j+1}) \\
     p_i(0,\sminus) &\le v_i(0,\sminus) 
\end{align*}
where $x_1 =0, x_2, \cdots, x_r \in S_i$ are the signals such that $f(\profile) = a_j$ for all $s_i \in [x_{j}, x_{j+1})$, and $a_1,\cdots, a_r$ as defined in Definition~\ref{defn:linear-single-crossing}.
\end{proposition}


%\subsection{Generalization of Strong Single Crossing 
\subsection{Beyond Welfare Maximization}
%\vspace{1ex}
%\noindent{\bf Beyond welfare maximization.}
\label{sub:linear-characterization}
The simple demonstration above also illustrates the fact that the strong single-crossing condition need not be limited to welfare maximization exclusively. To find the correct prices, it is sufficient to consider the regions at which each project gets allocated.
The fact that the project was chosen by maximizing welfare had been incidental to our process. This allows us to define the \emph{$f$-single-crossing condition}, which characterizes implementablity for any social choice function $f$ over \linear valuations.\footnote{This also holds for decomposable valuations. See Section~\ref{sec:decomposable}.} {\citet{JehieM01} define similar conditions for characterizing Bayesian incentive compatibility for fully linear valuations.\footnote{{Their conditions apply to multi-parameter signal spaces, but they coincide with $f$-single-crossing in the special case of single-parameter settings with fully linear valuations.}}}

\begin{definition}[$f$-single-crossing]\label{defn:linear-f-single-crossing}
 Given any IDV social choice setting $(n,\mathcal{S}, \mathcal{A},\vprofile)$ with \linear valuations $\vprofile$, and a (possibly randomized) social choice function $f$.
 We say that $\vprofile$ satisfies $f$-single-crossing, if for each $i\in [n]$ and $\sminus\in \mathcal{S}_{-i}$, and any signals $s_i < s'_i$
 \[
     f(s_i,\sminus) = a_1 , f(s'_i,\sminus) = a_2
 \]
 implies
 \[
    \pdif{v_i}{s_i}(a_1;\profile)\le \pdif{v_i}{s_i}(a_2;\profile) .
 \]
\end{definition}

\begin{observation}\label{obv:f-sc and strong-sc}
Let $\vprofile$ be an \linear valuation profile, and $f$ the welfare maximizing social choice function.
Then, $\vprofile$ satisfies $f$-single-crossing if and only if $\vprofile$ satisfies strong single-crossing.
\end{observation}

% \michal{The wording of the above observation is a bit unclear. How about the following: 
% Let $\vprofile$ be a decomposable valuation profile, and $f$ the welfare maximizing social choice function.
% Then, $\vprofile$ satisfies $f$-single-crossing if and only if $\vprofile$ satisfies strong single-crossing.
% }


% \dnote{Again, note that, for any \linear valuations $\vprofile$, we see that $\pdif{v_i}{s_i}{(a;\profile)}$ is a constant with respect to $s_i$. In particular, there exists functions $g_i: \mathcal{A}\times \mathcal S_{-i} \to \reals^+$ such that,
% \begin{align}
%     v_i(a;\profile) = s_i\cdot \pdif{v_i}{s_i}(a;\profile) + g_i(a;\sminus) \qquad \forall \profile \in \mathcal{S}, \; a \in \Delta(\mathcal{A}),\label{eq:decomposable-linear}
% \end{align}
% where both $\pdif{v_i}{s_i}(a;\profile)$ and $g_i(a;\sminus)$ don't depend on $s_i$. We will see this decomposability property is crucial to prove the following proposition.}

%\michal{Consider replacing the above paragraph with the following (I think we can restrict attention to a single valuation function rather than a valuation profile, please let me know if I'm wrong here): 

{For any \linear valuation function $v_i$,   $\pdif{v_i}{s_i}{(a;\profile)}$ is a constant. 
In particular, there exists a function $g_i: \mathcal{A}\times \mathcal S_{-i} \to \reals^+$ such that,
\begin{align}
    v_i(a;\profile) = s_i\cdot \pdif{v_i}{s_i}(a;\profile) + g_i(a;\sminus) \qquad \forall \profile \in \mathcal{S}, \; a \in \Delta(\mathcal{A}),\label{eq:decomposable-linear}
\end{align}
where neither  $\pdif{v_i}{s_i}(a;\profile)$ nor $g_i(a;\sminus)$ depends on $s_i$. This decomposability property is key in proving the following proposition.
}

\begin{proposition}\label{prop:linear-f-necessary}
For any IDV social choice setting with \linear valuations $\vprofile$, if a social choice {function} $f$ is ex-post truthfully implementable, then $\vprofile$ satisfies $f$-single-crossing.
\end{proposition}
\begin{proof}
Recall that $f$ is a ex-post truthfully implementable if for all $i\in [n]$ there exists a price function $p_i: \mathcal{S} \to \reals$ such that
\[
    \langle v_i(\profile), f(\profile)\rangle - p_i(\profile) \geq
    \langle v_i(\profile), f(s_i',\sminus)\rangle - p_i(s_i',\sminus) \qquad \forall \profile \in \mathcal{S}, \; \forall s'_i \in S_i.
\]
Similarly, when the true signal is $s_i'$ we have,
\[
    \langle v_i(s_i',\sminus), f(s_i',\sminus)\rangle - p_i(s_i',\sminus) \geq
    \langle v_i(s_i',\sminus), f(\profile)\rangle - p_i(\profile) \qquad \forall \profile \in \mathcal{S}, \; \forall s'_i \in S_i.
\]
Adding the above two inequalities and rearranging we get,
\begin{align}
    \langle v_i(\profile) - v_i(s_i',\sminus), f(\profile)\rangle  \geq
    \langle v_i(\profile)- v_i(s_i',\sminus), f(s_i',\sminus)\rangle  \qquad \forall \profile \in \mathcal{S}, \; \forall s'_i \in S_i.
\end{align}
Since $\vprofile$ is \linear, we note that $v_i(\profile) - v_i(s'_i,\sminus) = (s_i - s'_i)\pdif{v_i}{s_i}(\profile)$ by using the decomposition of $v_i$ from Eq.~\eqref{eq:decomposable-linear}. This implies, for all $i\in [n]$, $\sminus \in \mathcal{S}_{-i}$, and $s_i > s'_i \in S_i$ ,
\begin{align*}
    \langle (s_i - s'_i)\pdif{v_i}{s_i}(\profile), f(\profile)\rangle  &\geq
    \langle (s_i - s'_i)\pdif{v_i}{s_i}(\profile), f(s_i',\sminus)\rangle
\end{align*}
and therefore
\begin{align*}
    \langle \pdif{v_i}{s_i}(\profile), f(\profile)\rangle  &\geq
    \langle \pdif{v_i}{s_i}(\profile), f(s_i',\sminus)\rangle  
\end{align*}
Hence proving $\vprofile$ satisfies $f$-single-crossing.
\end{proof}



\subsection{Extension to Decomposable Valuations}\label{sec:decomposable}

%\michal{Perhaps the following paragraph can be shortened as follows: 

%In this section we show that our results for \linear valuations extend to a broader class of valuations. 
{Recall that the decomposition property 
of \linear valuations (Eq.~\ref{eq:decomposable-linear}) was key in enabling the characterization through $f$-single-crossing. 
With this in mind, we define a broader class of valuations called \emph{decomposable valuations} and  extend the  characterization found for \linear to this braoder class.

}

% In this section we show that our results for \linear valuations extend to a broader class of valuations. Recall that, the decomposition 
% of \linear valuations in Eq.~\ref{eq:decomposable-linear} is what enabled the characterization through $f$-single-crossing. With this in mind, we define a broader class of valuations called \emph{decomposable valuations} that gives a nice decomposition of $\vprofile$ that directly allows us to extend the characterization results beyond \linear.
% \michal{I noticed there is always a space after the multi-linear macro, and before comma, dots, etc. it should not be there}

For any decomposable valuation $v_i$, there exists a decomposition of $v_i(a;\profile) = \hat{v_i}(\profile)h_i(a;\sminus) + g_i(a;\sminus)$, where $\hat v_i: \mathcal{S} \to \reals^+$, $h_i: \mathcal{A}\times \mathcal{S}_{-i} \to \reals^+$, and $g_i: \mathcal{A}\times \mathcal{S}_{-i} \to \reals^+$.
It is easy to see that the class of decomposable valuations also contains \linear valuations, where for any linear valuation $v_i$ the corresponding $\hat v_i (\profile) = s_i$.

For any decomposable valuations $\vprofile$, we note that $\pdif{v_i}{s_i}(a;\profile) = h_i(a;\sminus)\pdif{\hat v_i}{s_i}(\profile)$. Thus, Definitions~\ref{defn:linear-single-crossing} and~\ref{defn:linear-f-single-crossing} can be immediately extended to decomposable valuations. 


\begin{observation}\label{obv:decomposable-ssc-fsc}
For any decomposable valuation $v_i$, we define \emph{strong single-crossing} and \emph{$f$-single-crossing} exactly like Definition~\ref{defn:linear-single-crossing} and Definition~\ref{defn:linear-f-single-crossing} respectively.
Further, for any decomposable valuation profile $\vprofile$ Observation~\ref{obv:f-sc and strong-sc} holds.
\end{observation}


Hence, by following the proof approach of Proposition~\ref{prop:linear-f-necessary} we immediately get that $f$-single-crossing is necessary {to truthfully implement $f$} for any IDV setting with decomposable valuations.


\begin{corollary}\label{cor:f-sc-necessary}
Given any IDV social choice setting with decomposable valuations $\vprofile$, a social choice function is truthfully implementable only if $\vprofile$ satisfies $f$-single-crossing. 
\end{corollary}


Moreover, we show that, for any decomposable valuation profile $\vprofile$, $f$-single-crossing is both necessary and sufficient condition for ex-post truthful implementability. {We defer the proof to the appendix.}

%\michal{I noticed that in some theorems we write interdependent values setting and in other s we write IDV setting. Would be good to be consistent.}

\begin{theorem}\label{thm:linear-characterization}
    For any IDV social choice setting with decomposable valuations $\vprofile$, a mechanism {$(f,p)$} is ex-post IC-IR  if and only if for every $i$, $\sminus$, $f$-single-crossing holds, and the following payment identity and payment inequality hold:
    \begin{align*}
        p_i(\profile) &= \; p_i(0,\sminus) + \int_{0}^{s_i} \left\langle v_i(t,\sminus), \pdif{f}{s_i}(t,\sminus) \right\rangle dt ;  \\
        p_i(0,\sminus) &\leq  \left\langle v_i(0,\sminus), f(0,\sminus) \right\rangle 
    \end{align*}
    
    Moreover, if we additionally require prices to be non-negative, it is sufficient to additionally have the following payment identity:
    %\begin{align}
    $
        p_i(0,\sminus) =  \left\langle v_i(0,\sminus), f(0,\sminus) \right\rangle
    $
\end{theorem}

==> arXiv version/prelims.tex <==
\section{Preliminaries}
\label{sec:prelim}

In this section we introduce notation for classic social choice %, public projects and single-parameter auction 
settings (Section~\ref{sub:prelim-IPV}) and define interdependent values (Section~\ref{sub:prelim-IDV}). %After presenting classic implementability results (Section~\ref{sub:prelim-IC-IPV}) 
We concisely summarize what's known in the literature about truthful implementation for interdependence (Section~\ref{sub:prelim-IC-IDV}; see Appendix~\ref{sub:prelim-IC-IPV} for truthful implementation \emph{without} interdependence). In Section~\ref{sub:prelim-PP} we present our main setting of interest -- public projects with interdependence.
%\michal{why single out the AGT literature? I see that we have there other results as well, such as Chung-Ely. How about just omit the words "in the AGT literature"?}

%\outline{Our model: public projects + IDV. Social welfare objective. Ex post IC. Truthful in expectation.}

\vspace{1ex}
\noindent{\bf Notation.}
For a vector $\mathbf{x}=(x_1,\ldots,x_n)$, we use the standard notation of $\mathbf{x}_{-i}$ to denote the same vector excluding $x_i$, and $(x'_i, \mathbf{x}_{-i})$ to denote the profile obtained by replacing $x_i$ with $x'_i$. %\inbal{Define the product notation.}

\subsection{Independent Private Values (IPV)}
\label{sub:prelim-IPV}

%\inbal{From meeting: It's not clear that single-dim is not a special case of PP; PP gets lost, we could have a subsection just on PP - Sec 2.4 with example of PP in IDV, with multi-linear valuations, say it's also decomposable valuations - instantiate the definitions and terms that we introduce. Take PP out of 2.1. Suggestion for restructure: leave 1st paragraph, then go to mechanism and truthfulness (including Def 2.1).}

\noindent{\bf Social choice settings.}
A social choice setting $(n,\mathcal{V},\mathcal{A})$ consists of $n$~\emph{agents} $\{1,\ldots,n\}$, a \emph{domain} of valuations $\mathcal{V}=V_1\times\ldots\times V_n$, and $\mu$ \emph{alternatives} $\mathcal{A}$ ($\mathcal{A}$ is also referred to as the \emph{outcome} space). In a particular instance, every agent~$i$ has a valuation function $v_i\in V_i$, %belonging to her space of possible valuations $V_i$; 
where function $v_i : \mathcal{A} \to \reals^+$
specifies her value for every alternative (we sometimes also use a vector notation $v_i \in \reals^\mu$). 
A \emph{social choice function} $f:\mathcal{V}\to\mathcal{A}$ maps a valuation profile to one of the alternatives, possibly randomized.
We denote by $f_a(\vprofile)$ the probability assigned to alternative $a\in\mathcal{A}$.
A \emph{finitely-valued} $f$ has finitely-many distinct outcomes, that is, for every $i\in [n]$ and $\vprofile_{-i}$, $|\{ f(v_i,\vprofile_{-i}): v_i \in V_i\}| < \infty$.  %\inbal{define}.
The \emph{welfare} of an alternative is the sum of the agents' values for it. 
%We say that the domain $\mathcal{V}$ is \emph{convex} if its closure is convex. \inbal{I think we should add details here}

\vspace{1ex}
\noindent{\bf Single-dimensional social choice settings.}
An important distinction is between settings with single- vs.~multi-dimensional domains. In the former,
the space $V_i$ is single-dimensional for every~$i$, i.e., there is a single real parameter that directly determines the valuation function $v_i$. %(see below). 
Such domains are well-known to be significantly simpler for mechanism design than multi-dimensional ones.

%\inbal{Should we remove ``auction'' from this setting's name?} 
Formally, a single-dimensional setting $(n,\mathcal{V},\mathcal{A})$ is a social choice setting in which the alternatives are subsets of agents, i.e., $\mathcal{A}\subseteq 2^{[n]}$. 
It is required that $\mathcal{A}$ be \emph{downward-closed} (if $W\in \mathcal{A}$ then for every $W'\subseteq W$, $W'\in \mathcal{A}$).
An outcome $W\in\mathcal{A}$ corresponds to a set of ``winning'' agents. For example, in a single-item auction, $\mathcal{A}=[n]$; in a multi-unit auction with $n$ units, $\mathcal{A}=2^{[n]}$. The valuations in such settings are simple:
%In these settings, the outcome space $\mathcal{A} \subseteq 2^{[n]}$ is a downward-closed subset, and the valuation functions can be defined as 
slighly overloading notation, every agent $i$ has a single value $v_i$ for winning, such that
$v_i(W)=v_i$ if $i \in W$, and $v_i(W)=0$ otherwise. We use $f_i(\vprofile)$ to denote the probability that agent $i$ is a winner.

\vspace{1ex}
\noindent{\bf Mechanisms.}
A (direct revelation) mechanism solicits value reports $\mathbf{b} =(b_1,\ldots,b_n)$ from the agents. Its description is given by a pair $(f,p)$, where $f$ is a social choice function, and $p$ a collection of payment rules $p(\mathbf{b})=\{p_1(\mathbf{b}), \ldots, p_n(\mathbf{b})\}$.
Payment rule $p_i: \mathcal{V} \to \reals$ maps the bids $\mathbf{b}$ to the expected payment of agent $i$. For every $i$, agent $i$'s expected quasi-linear utility is given by 
$\sum_{a\in \mathcal{A}} f_a(\mathbf{b}) v_i(a) - p_i(\mathbf{b})$. We sometimes use an inner product  $\langle v_i, f(\mathbf{b})\rangle$ to denote $\sum_{a\in \mathcal{A}} f_a(\mathbf{b}) v_i(a)$.
%$\sum_{j=1}^m f_j(\mathbf{b}) v_i(j; \profile) - p_i(\profile)$ where $\profile$ is the true signal profile of the agents.

\vspace{1ex}
\noindent{\bf Truthfulness and implementability.}
Truthfulness is without loss of generality by the revelation principle~\citep{Myerson1981}.
For standard IPV settings, we focus on the design of dominant-strategy incentive-compatible (IC) and individually rational (IR) mechanisms: 
A {deterministic} mechanism is considered \emph{truthful} if it is in every agent's best interest to participate and report her true value \emph{regardless of others' bids} (bidding truthfully is a dominant-strategy equilibrium of the mechanism).
%In interdependent settings, we cannot hope to design mechanisms where truth-telling is a dominant strategy, therefore incentive compatibility (IC) and individual rationality (IR) are defined \emph{ex-post}, i.e., it is in every bidder's best interest to participate and report her true signal \emph{given that all other bids are also truthful} (bidding truthfully is an ex-post equilibrium of the mechanism).
Formally, a {deterministic} mechanism is dominant-strategy IC-IR if 
for every valuation profile $\vprofile\in \mathcal{V}$, agent $i\in[n]$ and bid $b_i\in V_i$,
\[
    \sum_{a\in\mathcal{A}} f_a(\vprofile) v_i(a) - p_i(\vprofile) \geq \max\Big\{ \sum_{a\in\mathcal{A}} f_a(b_i,\vprofile_{-i}) v_i(a) - p_i( b_i,\vprofile_{-i}), 0\Big\}. 
\]
%The following definition plays a central role in our results:

%\michal{The aboev definition is for truthful in expectation, isn't it?}

For randomized mechanisms there are two levels of truthfulness: the mechanism can be truthful for every realization of its internal randomness, in which case we say it is \emph{universally truthful}; a weaker requirement is that the mechanism is  \emph{truthful in expectation} where the expectation is taken over its random coins. Unless stated otherwise, by ``truthful'' we refer to the former requirement of universal truthfulness. %\inbal{Did we want to say which we mean by default?}
%\inbal{Either strengthen our impossibility result for truthful in expectation or state this as an open problem.}

\begin{definition}
\label{def:implementable}
Consider a social choice setting $(n,\mathcal{V},\mathcal{A})$.
A social choice function $f$ is called \emph{implementable} if there exists a payment rule $p$ such that $(f,p)$ is truthful.
\end{definition}


\subsection{Interdependent Values (IDV)} 
\label{sub:prelim-IDV}

Our focus in this work is on the \emph{interdependent} values (IDV) model of \citet{MW82}. In the standard independent private values (IPV) model, the privately-known \emph{type} of each agent $i$ is her valuation~$v_i$. In IDV, however, the privately-known type is her \emph{signal} $s_i$, which captures her information on the social choice alternatives.%
\footnote{Note that this makes the types in our model -- despite its possible combinatorial nature -- single-parameter. We emphasize this does not mean that interdependent settings are always single-dimensional, rather that the dimensionality of the type is distinct from that of the setting.}
Formally, let the set of possible signals $S_i$ be $[0,1]$ for every agent $i\in[n]$. 
%receives a single private signal $s_i$. 
We denote by $\profile=(s_1,s_2,\ldots,s_n)$ a signal profile, and by $\mathcal{S} = \times_i S_i$ the signal space of the agents.
%The set of potential signals for agent $i$ is denoted $S_i$, for each $i\in\{1,\ldots,n\}$. Unless stated otherwise, we use $S_i = [0,1]$ for all $i\in\{1,\ldots,n\}$ throughout the paper.
The \emph{values} of the agents are interdependent in the following sense: they depend not only on the chosen alternative $a\in\mathcal{A}$, but also on the information (signals) of all the agents. That is, for every $i$, the valuation function of agent $i$ is $v_i: \mathcal{A}\times \mathcal{S} \rightarrow \reals^+$ (we sometimes also denote $v_i(\cdot; \profile)$ as $v_i(\profile) \in \reals^\mu$ where the alternative $a$ is clear from the context). %(that is, for \emph{additive} public projects $v_{i}(j,\profile) = v_{ij}(\profile)$ for all $j\in [m]$).
We assume (as is standard) that for every pair $i,i'\in[n]$, valuation $v_i$ is monotone non-decreasing in signal $s_{i'}$ . 
The collection of valuation functions $\vprofile=\{v_i\}_i$ is publicly known.

\vspace{1ex}
\noindent{\bf Social choice with IDV.}
Classic social choice settings can be adapted to IDV with only slight changes (mainly, $\profile$ replacing $\vprofile)$: A social choice setting with IDV $(n,\mathcal{S},\mathcal{A},\vprofile)$ consists of $n$ agents, a signal space~$\mathcal{S}$, alternatives $\mathcal{A}$, and a profile of $n$ valuation functions $v_i: \mathcal{A}\times \mathcal{S} \rightarrow \reals^+$. 
We refer to such settings as interdependent values (IDV) settings or as social choice settings with IDV.
A social choice function $f: \mathcal{S} \rightarrow \mathcal{A}$ maps each signal profile $\profile$ to a (possibly random) social alternative. For any distribution over outcomes $\delta \in \Delta(\mathcal{A})$,  we use $v_i(\delta; \profile)$, $\langle v_i(\profile) , \delta\rangle$, and $\sum_{a\in \mathcal{A}}\delta(a)v_i(a;\profile)$ interchangeably to denote agent $i$'s expected value.
%The rest of the setup mirrors that of a classic social choice setting. 
A %combinatorial public projects or 
single-dimensional setting with IDV is similarly defined. For simplicity, in single-dimensional settings we often omit the alternative from the valuation function notation, and let $v_i:\mathcal{S} \rightarrow \reals^+$ be such that $v_i(a; \profile)=v_i(\profile)$ if $i \in a$ (agent $i$ wins), and $v_i(a; \profile) = 0$ otherwise.
%\michal{Why do we have auctions in the title of this paragraph? also, why in the last line the domain is $\mathcal{S}$ rather than $\mathcal{A}\times \mathcal{S}$?}

\vspace{1ex}
\noindent{\bf Subclasses of interdependent valuations.} 
%\inbal{What do you think of using ``multilinear'' instead of ``linear''? It's more precise I think}
An important subclass of interdependent valuations are \emph{\linear}valuations. A valuation $v_i$ is \linear if for every $a$ and $\profile_{-i}$, $v_i(a; s_i, \profile_{-i})$ is linear as a function of $s_i$. This class encompasses well-studied special cases like the resale model~\citep{Myerson1981,RT16,EdenFTZ21} or Klemperer’s wallet game~\citep{Klemperer1998}.

%\inbal{separable valuations. Find the source -- mookherjee.}

%\vspace{1ex}
%\noindent{\bf Decomposable valuations.} 
We introduce the following 
natural extension, which distills the essence of \linear valuations and serves as the domain of our main results. We say that a valuation $v_i$ is decomposable if there exist functions $\hat v_i : \mathcal{S} \to \reals^+$, $h_i : \mathcal{A}\times \mathcal{S}_{-i} \to \reals^+$ and $g_i: \mathcal{A}\times \mathcal{S}_{-i} \to \reals$, such that for every $a,\,\profile$ we have 
\begin{equation}
v_i(a;\profile) = \hat{v}_i(\profile)\cdot h_i(a;\sminus) + g_i(a;\sminus).\label{eq:decomp}
\end{equation}

For example, the valuation function $v_1$ defined as $v_1(1;\profile) = s_1^2 + s_2$, $v_1(2;\profile) = s_1^2s_2$ is a decomposable valuation, where $\hat{v}_1(s_1,s_2) = s_1^2$, $h_1(1;s_2) = 1 ,h_1(2;s_2) = s_1$, $g_1(1;s_2) = s_2$, and $g_1(2;s_2)=0$.

We observe that decomposable valuations are strictly more general than the following classes of valuations: (i) separable\footnote{Not to be confused with separable SOS, as defined in~\citep{EFFGK19} -- see Section~\ref{sec:approximation}.} environments{~\citep{MookherjeeR92,CE02}}, where $h_i$ does not depend on $\sminus$ and $g_i \equiv 0$, (ii) single-dimensional settings,  where $h_i(a;\sminus) = 1$ if $i\in a$ and $0$ otherwise and $g_i\equiv 0$, and (iii) \linear valuations where $\hat v_i(s_i,\sminus)=s_i$. 


% \begin{definition}
% \dnote{Given any IDV setting $(n,\mathcal{S},\mathcal{A},\vprofile)$, for each $i$, $\sminus$, let $V_i(\sminus) = \{v_i(\profile)\in \reals^\mu| \forall s_i \in S_i\}$. We say that the domain is convex if the closure of $V_i(\sminus)$ is convex for each $i$ and $\sminus$.}
% \end{definition}

% \inbal{Need to add here a definition of a domain, convexity of the domain, and dimension of the domain.}\divya{maybe it's not needed here, can move it to section 3.2?}
%The project selection function $f$ maps a signal profile $\profile$ to a vector as follows: $f(\profile)=(f_1(\profile),\ldots, f_m(\profile))$, where $f_j(\profile)\in[0,1]$ is the probability that project $j$ is chosen. 
%If the allowed number of projects is $k$,
%such that $\sum_i f_i(\profile) \leq 1$ holds for all possible $\mathbf{b}$, \avi{actually this should be 
%then $\sum_{j=1}^m f_j(\profile) \leq k$. %for every $\profile$. %and $f_i(\profile)\leq 1$ for $i\in[m]$ in the general $k\geq1$ project setting. %A social choice function $f_i: \mathcal{S} \to [0,1]$ maps every bid profile $\mathbf{b}$ to the probability that project $i$ gets chosen.
%In these settings, the outcome space $\mathcal{A} \subseteq 2^{[n]}$ is a downward-closed subset, and the valuation functions can be defined as $v_i:\mathcal{S} \rightarrow \reals^+$ (i.e., $v_i(a; \profile) = v_i(\profile)$ if $i \in a$, and $v_i(a; \profile) = 0$ otherwise). We use $f_i(\profile)$ to denote the probability that agent $i$ is allocated the item.

\vspace{1ex}
\noindent{\bf Mechanisms and truthfulness with IDV.}
A mechanism for IDV solicits signal rather than value reports $\mathbf{b} =(b_1,\ldots,b_n)$ from the agents. %Its description is given by a pair $(f,p)$, where $f$ is a social choice function, and $p$ a collection of payment rules $p(\mathbf{b})=\{p_1(\mathbf{b}), \ldots, p_n(\mathbf{b})\}$.
%Payment rule $p_i: \mathcal{S} \to \reals$ maps the reported bids $\mathbf{b}$ to the expected payment of agent $i$. 
For every $i$, agent $i$'s expected quasi-linear utility is given by 
$\sum_{a\in A} f_a(\mathbf{b}) v_i(a; \profile) - p_i(\mathbf{b})$.
%$\sum_{j=1}^m f_j(\mathbf{b}) v_i(j; \profile) - p_i(\profile)$ where $\profile$ is the true signal profile of the agents.
%We focus on the design of incentive-compatible and individually rational mechanisms (this is without loss of generality by the revelation principle~\cite{Myerson1981}). 
In interdependent settings, it is well-known that we cannot hope to design mechanisms where truth-telling is a dominant strategy, therefore incentive compatibility and individual rationality are defined \emph{ex-post}. I.e., a mechanism for IDV is considered \emph{truthful} if it is in every bidder's best interest to participate and report her true signal \emph{given that all other agents bid truthfully} (i.e., bidding truthfully is an ex-post equilibrium of the mechanism).
Formally, a deterministic mechanism is ex-post IC-IR if for every signal profile $\profile\in\mathcal{S}$, agent $i\in[n]$ and bid $b_i\in S_i$,
\[ 
    \sum_{a\in \mathcal{A}} f_a(\profile) v_i(a; \profile) - p_i(\profile) \geq \max\Big\{ \sum_{a\in \mathcal{A}} f_a(b_i,\profile_{-i}) v_i(a;\profile) - p_i( b_i,\profile_{-i}), 0\Big\},
\]
where $f_a(\profile)$ indicates whether alternative $a$ is chosen given $\profile$.
As above, a randomized mechanism is universally truthful if it consists of a distribution over truthful deterministic mechanisms. %rule i \divya{change this to deterministic social choice function and then define universally truthful}

\subsection{Implementability with IDV: What's Known}
\label{sub:prelim-IC-IDV}

In Appendix~\ref{sub:prelim-IC-IPV} we include several known key results on implementability for IPV. For IDV, implementability is more subtle, as we now detail.

\vspace{1ex}
\noindent{\bf Single-dimensional settings.}
%\outline{Single crossing for auctions. Implementability for auctions (and the kind of single crossing it implies -- possibly say that for linear this coincides with ``slope'' single crossing). Reduction from single-item auctions to public projects.} %SOS and impossibility without it.}
%In this section we discuss certain well-studied properties and definitions in auction design with interdependent values. 
For single-dimensional settings with IDV, monotonicity characterizes implementable social choice functions (similarly to IPV). Recall that %for a given social choice function $f$ and signal profile $\profile$, we denote by 
$f_i(\profile)$ denotes the probability that agent~$i$ wins. Then:

\begin{theorem}[Implementability with IDV: Single-dimensional~(e.g.~\citep{RT16})]\label{thm:single-dim-charaterization}
For every single-dimensional IDV setting, a social choice function $f$ is (ex post IC-IR) implementable if and only if for every $i,\sminus$ 
it holds that $f_i(s_i,\sminus)$ is monotone non-decreasing in signal~$s_i$. %~\cite{Myerson1981}.
%$f_i$ is monotone non-decreasing in the signal $s_i$.
\end{theorem}

Unlike IPV, it turns out that even to implement a social choice function like welfare maximization, with IDV an additional \emph{single-crossing} condition is needed in order to achieve monotonicity and hence truthfulness. %This well-known condition is called  condition is necessary (and sufficient) to maximize welfare in single-dimensional settings because it precisely gives the \emph{monotonicity} needed for truthfulness.
%\inbal{talk about that it comes up in social choice too}
Many definitions for such a condition appear in the literature, the following is adapted from~\citep{RT16}: %) is for single dimensional settings (such as single-item auctions, or multi-unit auctions with unit-demand buyers).   %\divya{ There was no single crossing for multi-dim before right? Should we rename "our" single-crossing as "general single-crossing" or something?}

\begin{definition}[Single-crossing condition]\label{def:sc-auctions}
Given a single-dimensional setting with IDV, we say that the valuation profile $\vprofile$ satisfies \emph{single-crossing} if for all agents $i,j$ and every  $ \profile \in \mathcal{S}$,
 $
    \pdif{v_i}{s_i}(\profile) \ge \pdif{v_j}{s_i}(\profile)
 $.
\end{definition}
%
\noindent That is, agent $i$'s signal influences her own valuation more than the valuation of any other agent. %\inbal{Explain why this is called single-crossing and what in general is the essence of a single crossing condition.}
%Refer to~\citep{RT16} for a more detailed study on characterizing truthfulness in single-dimensional setting with IDV.
%\divya{This also goes through because of Myerson + Chung-Ely?}
%\avi{How about the following explanation?:}
%The name single-crossing comes from the fact that for any $i$ and $j$ such that the inequality of the single-crossing condition holds, the curves $v_i(\cdot,\sminus)$ and $v_j(\cdot,\sminus)$ as a function of $s_i$ may only intersect once. This guarantees that for any pair of signals $s<s'\in S_i$ such that $v_i(s, \sminus) \geq v_j(s, \sminus)$ it must hold that $v_i(s', \sminus) \geq v_j(s', \sminus)$. That is, as we increase the signal $s_i$, the value of agent $i$ cannot go from being the top value to being below the value of some other agent $j$. In other words, the welfare maximizing allocation must be monotone.
This definition or slight variations of it in effect characterize truthfulness,
%\begin{lemma}[Welfare maximization with IDV]\label{lem:single-dim-welfare}
as for every single-dimensional setting with IDV, %there is an (ex post IC-IR) implementable mechanism that achieves optimal social welfare 
welfare maximization is implementable
if and only if the valuation profile $\vprofile$ satisfies single-crossing.
%\michal{is it right to use the word implementable here? isnt it simply an ex-post IC-IR mechanism? I thought implementable refers to social choice functions not mechanisms.}
%\end{lemma}

%\noindent{\bf Social choice implementability: From IPV to IDV.} %Background: Multi-dimensional mechanism design  (with IPV)}

%\subsection{Background: Connections between truthfulness in IPV and IDV}

\vspace{1ex}
\noindent{\bf Beyond single-dimensional settings.}
For settings beyond single-dimensional, there is a characterization for the following class in the context of welfare maximization:
%Generalizing single-dimensional settings, 
When the valuation functions are separable,~\citet{CE02} define a strengthened single-crossing condition that is necessary and sufficient for welfare maximization. 
Similar single-crossing conditions have appeared in the welfare maximization context under varying assumptions~\citep[e.g.,][]{DM2000,ItoP06,RobuPIJ13}. %\inbal{from meeting: add citations to dasgupta-maskin and parkes and check this sentence}.
We shall define a generalization of this condition in Definition~\ref{defn:linear-single-crossing} for the broader class of decomposable valuations, and apply it beyond welfare maximization.

%\vspace{1ex}
%\noindent{\bf General social choice settings.} 
To our knowledge, there is no generalized single-crossing condition that characterizes welfare maximization implementability in \emph{general} social choice settings with IDV.
However, \citet{CE02} establish a relationship between characterizing implementability in social choice settings with IDV and with IPV:

\begin{lemma}[Characterizing Implementability with IDV vs.~IPV, \citep{CE02}]
\label{lem:Chung-Ely}
%\inbal{Please check}
Let $C$ be a condition that applies to a quadruple $(\mathcal{A}, S, v(\cdot), f)$ that represents a single-agent, single-dimensional social choice setting with alternative set $\mathcal{A}$, value domain $\{v(s)\mid s\in S\}$, and a social choice function $f$.
The following characterizations using condition $C$ are equivalent, i.e., one holds if and only if the other holds.% exists if and only if the other exists:
\begin{itemize}
    %\item In the single-agent special case, the public decision rule $g:\Theta \to A$ is incentive compatible if (resp. only if) the quadruple $(A, \Theta, v, g)$ satisfies $C$.
    \item In a social choice setting with IDV, a social choice function $f : \mathcal{S} \rightarrow \mathcal{A}$ is ex post IC if (respectively only if) $\forall i, \forall s_{-i}$, the quadruple $(\mathcal{A}, S_i, v_i(\cdot~; s_{-i},\cdot), f( s_{-i},\cdot))$ satisfies condition $C$;
    \item %\inbal{Please check since I changed the notation} 
    In a social choice setting with IPV, social choice function $f : \mathcal{V} \rightarrow \mathcal{A}$ is dominant-strategy IC if (respectively only if) $\forall i, \forall s_{-i}$, the quadruple $(\mathcal{A}, V_i, v_i, f(s_{-i},\cdot))$ satisfies condition $C$.
\end{itemize}
\end{lemma}

\subsection{Interdependent Public Projects}
\label{sub:prelim-PP}

%\vspace{1ex}
%\noindent{\bf Combinatorial public projects settings.} 
A classic \emph{combinatorial public projects setting} $(n,\mathcal{V},m,k)$ is a multi-dimensional social choice setting in which there are $n$ agents, $m$ projects $\{1,\ldots,m\}$, and a number $k\le m$, $k \in \mathbb{N}$. 
The alternatives are all combinations of up to $k$ projects, i.e., $\mathcal{A}=\{T\subseteq[m]\mid |T| \le k\}$.
A combinatorial public projects setting \emph{with interdependent values} is described by $(n,\mathcal{S},\vprofile,m,k)$, and the value of agent $i$ for project set $T$ is $v_i(T,\profile)$. 
%In a particular instance, each agent has a valuation function $v_i : 2^{[m]} \to \reals^+$ over subsets of projects. %The set $V_i$ denotes the space of possible valuations of agent $i$, and $\mathcal{V}$ denotes the \emph{domain} of valuations $V_1\times\ldots\times V_n$.
%We sometimes refer to the social choice function in the context of public projects as the \emph{project selection function}. 
%Let $f_j(\vprofile)\in[0,1]$ be the probability that project $j\in[m]$ is chosen. 
In the combinatorial public projects \emph{problem (CPPP)}, the input is a public projects setting and the objective is to find a subset $T^*$ of up to $k$ projects that maximizes the social welfare: $T^*\in \arg\max_{T\in\mathcal{A}}\sum_{i=1}^n v_i(T,\profile)$.
%\inbal{Please check the previous paragraph and the next one}
%\divya{This is not enough in general, because the rounding can be ``infeasible''. It is better to consider $\mathcal{A} = {[m] \choose \le k}$.}

In the following example, the valuation of agent~1 is \linear while the valuation of agent~2 is not \linear (since $v_{22}$ depends on $(s_2)^2$) but is decomposable, and the valuation of agent~3 is not even decomposable (since $v_{31}$ and $v_{32}$ depend on $s_3$ in different ways -- recall Eq.~\eqref{eq:decomp}). %\inbal{Add a 1-sentence explanation} %For completeness in Example~\ref{ex:non-example} we show a setting in which the valuation of agent ... is non-decomposable. 

\begin{example}[Public project instance with interdependence]
There are $n=3$ agents and $m=2$ projects. Assume $k=1$, i.e., a single project can be realized. 
Each signal space is $\{0, 1, 2\}$, and the valuations of the agents for the two projects depend on the signals as follows:
\begin{itemize}
    \item \textbf{Agent 1: \Linear.} $v_{11}=s_1s_2$, $v_{12}=s_1({s_2})^2$;
    \item \textbf{Agent 2: Decomposable.} $v_{21}=s_1 + (s_2)^2$, $v_{22}=s_1({s_2})^2$;
    \item \textbf{Agent 3: Non-decomposable.} $v_{31}=s_1 + s_2 + s_3$, $v_{32} = s_1(s_3)^3$.
\end{itemize}
Analysis: Under signal profile $(1,0,0)$, the welfare-maximizing project is project~1 (with social welfare of $2$, compared to a social welfare of $0$ for the other project). Under signal profile $(1,2,2)$, the welfare-maximizing project is project~2 (with social welfare of $16$, compared to a social welfare of $12$ for the other project). 
\end{example}

